Navigating the Pitfalls of Active Learning Evaluation: A Systematic Framework for Meaningful Performance Assessment

Active Learning (AL) aims to reduce the labeling burden by interactively selecting the most informative samples from a pool of unlabeled data. While there has been extensive research on improving AL query methods in recent years, some studies have questioned the effectiveness of AL compared to emerging paradigms such as semi-supervised (Semi-SL) and self-supervised learning (Self-SL), or a simple optimization of classifier configurations. Thus, today's AL literature presents an inconsistent and contradictory landscape, leaving practitioners uncertain about whether and how to use AL in their tasks. In this work, we make the case that this inconsistency arises from a lack of systematic and realistic evaluation of AL methods. Specifically, we identify five key pitfalls in the current literature that reflect the delicate considerations required for AL evaluation. Further, we present an evaluation framework that overcomes these pitfalls and thus enables meaningful statements about the performance of AL methods. To demonstrate the relevance of our protocol, we present a large-scale empirical study and benchmark for image classification spanning various data sets, query methods, AL settings, and training paradigms. Our findings clarify the inconsistent picture in the literature and enable us to give hands-on recommendations for practitioners. The benchmark is hosted at https://github.com/IML-DKFZ/realistic-al .

==> tables/cifar100_high.tex <==
\begin{tabular}{llllllll}
\multicolumn{4}{l}{Information}             & \multicolumn{4}{l}{Number Labeled Training Samples} \\
Paper         & Method  & Model    & Source & 5k          & 10k         & 15k        & 20k        \\
Munjal et al. & SL      & VGG16    & Graph  & 39,44       & 49          & 55         & 59         \\
Munjal et al. & SL      & ResNet18 & Table  & ?           & 61,06       & 66,92      & 69,83      \\
Mittal et al. & SL      & WRN28-2  & Graph  & 44,9        & 58          & 64         & 68         \\
Mittal et al. & Semi-SL & WRN28-2  & Graph  & 59          & 65          & 70         & 71         \\
Bengar et al. & SL      & ResNet18 & Graph  & 27          & 45          & 52         & 58         \\
Bengar et al. & Self-SL & ResNet18 & Table  & 60          & 63          & 63,5       & 64         \\
Gao et al.    & Semi-SL & WRN28-2  & Table  & 63,35       & 67          & 68         & 70         \\
Ours          & SL      & ResNet18 & Table  & 49,16       & 61,25       & 66,72      & 70,25      \\
Ours          & Self-SL & ResNet18 & Table  & 60,36       & 64,77       & 68,37      & 70,71     
\end{tabular}

==> tables/cifar100_low-med.tex <==
\begin{tabular}{llllllll}
\multicolumn{4}{l}{Information}             & \multicolumn{4}{l}{Number Labeled Training Samples} \\
Paper         & Method  & Model    & Source & 500         & 1000        & 2000       & 2500       \\
Mittal et al. & SL      & WRN28-2  & Graph  & 9           & 12          & 24         & 34         \\
Mittal et al. & Semi-SL & WRN28-2  & Graph  & 26          & 35,5        & 44,5       & 49         \\
Bengar et al. & SL      & ResNet18 & Graph  & 9           & 12          & 17         & -          \\
Bengar et al. & Self-SL & ResNet18 & Table  & 47          & 50          & 56         & -          \\
Ours          & SL      & ResNet18 & Table  & 14,03       & 22,39       & 31,99      & 36,27      \\
Ours          & Self-SL & ResNet18 & Table  & 37,32       & 45,22       & 52,16      & 54,71      \\
Ours          & Semi-SL & ResNet18 & Graph  & 37,5        & -           & 54,5       & -         
\end{tabular}

==> tables/cifar10_high.tex <==
\begin{tabular}{llllllll}
\multicolumn{4}{l}{Information}                         & \multicolumn{4}{l}{Number Labeled Training Samples} \\
Paper           & Method  & Model       & Source        & 5k          & 10k         & 15k        & 20k        \\
QBC             & SL      & DenseNet121 & Munjal et al. & 74          & 82,5        &            &            \\
VAAL            & SL      & VGG16       & Munjal et al. & 61,35       & 68,17       & 72,96      & 75,99      \\
CoreSet         & SL      & VGG16       & Munjal et al. & 60          & 68          & 71         & 74         \\
Munjal-SR       & SL      & VGG16       & Munjal et al. & 82,16       & 85,07       & 89,43      & 91,16      \\
LLAL            & SL      & ResNet18    & Munjal et al. & 81          & 87          & -          & -          \\
CoreCGN         & SL      & ResNet18    & Munjal et al. & 80          & 85,5        & -          & -          \\
TA-VAAL         & SL      & ResNet18    & Munjal et al. & 81          & 87,5        & -          & -          \\
Munjal-SR       & SL      & ResNet18    & Munjal et al. & 84,69       & 88,45       & 89,98      & 92,29      \\
Mittal et al.   & SL      & WRN28-2     & Graph         & 82,5        & 86          & 90,7       & 92         \\
Mittal et al.   & Semi-SL & WRN28-2     & Graph         & 92,5        & 93,8        & 94         & 94,5       \\
Bengar et al.   & SL      & ResNet18    & Graph         & 73          & 81          & 85         & 88         \\
Bengar et al.   & Self-SL & ResNet18    & Graph         & 89,5        & 90,5.       & 91         & 91,5       \\
Yi et al.       & SL      & ResNet18    & Graph         & 78          & 86          & -          & -          \\
Krishnan et al. & SL      & ResNet18    & Graph         & 78          & 86          & -          & -          \\
Ours            & SL      & ResNet18    & Table         & 85,50       & 90,50       & -          & -          \\
Ours            & Self-SL & ResNet18    & Table         & 90,05       & 91,40       & -          & -         
\end{tabular}


==> tables/cifar10_low.tex <==
\begin{tabular}{lllllll}
\multicolumn{4}{l}{Information}             & \multicolumn{3}{l}{Number Labeled Training Samples} \\
Paper         & Method  & Model    & Source & 50              & 100             & 200             \\
Bengar et al. & Self-SL & ResNet18 & Graph  & 62              & 77              & 81              \\
Gao et al.    & Semi-SL & WRN28-2  & Table  & -               & 47,85           & 89,20           \\
Ours          & SL      & ResNet18 & Table  & 25,14           & 32,33           & 44,36           \\
Ours          & Self-SL & ResNet18 & Table  & 71,31           & 76,80           & 81,18           \\
Ours          & Semi-SL & ResNet18 & Graph  & 90              & 91              & 93             
\end{tabular}

==> tables/cifar10_med.tex <==
\begin{tabular}{llllllll}
\multicolumn{4}{l}{Information}               & \multicolumn{4}{l}{Number Labeled Training Samples} \\
Paper           & Method  & Model    & Source & 250         & 500         & 1000       & 2000       \\
Mittal et al.   & SL      & WRN28-2  & Graph  & 36          & 48          & 57         & 73         \\
Mittal et al.   & Semi-SL & WRN28-2  & Graph  & 82          & 85          & 88         & 91         \\
Bengar et al.   & SL      & ResNet18 & Graph  & -           & 38          & 45         & 55         \\
Bengar et al.   & Self-SL & ResNet18 & Graph  & 83          & 85          & 87         & 88         \\
Yi et al.       & SL      & ResNet18 & Graph  & -           & -           & 47,5       & 56         \\
Krishnan et al. & SL      & ResNet18 & Graph  & -           & -           & 47         & 60         \\
Gao et al.      & Semi-SL & WRN28-2  & Graph  & 90,23       & -           & 92,5       & 92,5       \\
Ours            & SL      & ResNet18 & Table  & 46,95       & 61,15       & 72,38      & 79,83      \\
Ours            & Self-SL & ResNet18 & Table  & 81,41       & 84,13       & 86,22      & 88,26      \\
Ours            & Semi-SL & ResNet18 & Graph  & 93          & 94          & 94,5       & 95        
\end{tabular}

==> tex/99_depr_tex/02_OLD_relworks.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=.75\linewidth]{deep-active-plots/concept/deep_active-comp.pdf}
%     \caption{Caption}
%     \label{fig:relworks}
% \end{figure}

% \begin{wrapfigure}{l}{0.6\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/concept/deep_active-comp.pdf}
%     \caption{Test}
%     \label{fig:relworks}
% \end{wrapfigure}

% \begin{wrapfigure}{l}{0.6\linewidth}
%     \centering
%     \begin{adjustbox}{width=1.1\linewidth} 
%         \input{tables/main-comparison}
%     \end{adjustbox}
%     \makeatletter\def\@captype{table}\makeatother% "Change float to table"
%     \caption{Caption}
%     \label{tab:relworks}
% \end{wrapfigure}

\begin{table}[]
    \centering
    \begin{adjustbox}{width=\linewidth} 
    \input{tables/main-comparison}
    \end{adjustbox}
    \caption{Comparison of the evaluations in the Active Learning literature with regard to the setting values we propose to evaluate. Each of these papers should be viewed as stepping stone with useful insights based upon which we built our proposed evaluation.}
    \label{tab:relworks}
\end{table}

% whats special about AL eval? what makes it realistic?
% maybe validation paradox here? (how invasive in intro?)
% and the goals of evaluation
% state that we identified 5 key parameters that define realistic evaluation
% state that we will contrast the current state and related pitfals against our proposed improvement in all 5 topics.
%

%Realistic evaluation in AL is particularly tricky due to a phenomenon we refer to as the \textit{validation paradox}: AL parameters can not be configured on a new data set without directly contradicting the purpose of reducing labeling efforts. Thus, AL application, by definition, implies pre-configured methods to be rolled-out on new data sets. Realistic evaluation needs to reflect these circumstances and test AL methods 1) under a broad range of potential future data and label scenarios and 2) for generalizability of fixed configurations when rolled out on new data sets. Failure mode: cold start problem..

% Exact Recipes: how to work against validation paradox + K4K5
% default: test all the spectra: possible results agnosticity or only one fixed setting
% Exception: special task interest, limit spectrum
% could also guess fixed setting but not recomended way
% K4 K5 can be tuned on the data set upon applicaiton. Pitfall: statement "QM works" conditioned (K4, K5). Change K4, K5 can lead to drops on new data set because statement under new condition not been tested.
% K4 K5 important because statement is conditioned on them.
% How do we deal with K4 K5 interacting with QM? Not at all. -> Blindflug
% QM auf neuem dataset does not work. consequence of evaluation not according to our recipe. "aktiv entgegenwirken" - >K1-K3 wegen generalisierung, als K4K5 anpassen auf neues dataset. 
% Story K3: first did not test the spectrum (only fixed ratio starting budget zu K3. common practice get K3 from K2), We saw this was not good enough! Ran extra tests on smaller K3, saw BALD gets more robust.
% Batch Bald simuliert kleinere K3, "Batch Bald works" = "Bald works on small K3".

% Naming: Current pitfalls: .... Proposed improvement:

In this work, we make several improvements over the standard evaluation for deep active classification, which typically follows defined canonical steps:
First, a commonly available dataset used for supervised learning is split into an unlabeled pool dataset and small labeled initial dataset. As a successive training step, an arbitrary and not necessarily standardized model is then fitted on the small labeled dataset. The resulting trained model is then employed in conjunction with a query method to select a fixed amount of samples (defined by the query size) from the pool, which are labeled and added to the labeled dataset as an acquisition step. Finally, the performance of the model and query method pair is tracked over multiple acquisition steps, successively increasing the query size. Based on the results, a recommendation with regard to which query method is `best' then given.
\\
The choice of dataset, initial small labeled dataset size, and acquisition steps are to a large extend standardized across different papers. However, to our knowledge, it is never fully explained or ablated \textbf{\emph{why}} exactly these standardized settings are chosen. In theory, AL heavily dependents on these settings, which are often considered to be given but potentially vary greatly in practice for new datasets and different sampling strategies.\\ 

Further, the acquisition step itself depends on the training dataset, final model (which per se depends on the validation set and hyperparameters), unlabeled pool and query size. If these dependencies interact in an unfortunate manner, the \textit{cold-start problem} can occur, the event when an AL strategy performs worse than random queries. Commonly this phenomenon is observed on small initial datasets and for uncertainty based AL strategies understood as the situation where a ``bad model queries useless samples''. Therefore having a clear understanding of how the dependencies of the acquisition step interact and how to set up a well generalizing AL strategy is crucial for a successful application of AL.\\

The importance of these factors is further emphasized by taking into account the \textit{validation paradoxon}, stating that in a model-employed setting it is not without large difficulty to measure the change in performance through AL compared to random queries without including large additional labeling effort (whose reduction the purpose of AL is).\\
% \paragraph{Cold-Start Problem} Is commonly attributed when AL strategies perform (much) worse than random sampling (usually at early stages of the AL cycle and small starting budgets). This phenomena is mostly understood for uncertainty based acquisition with high acquisistion sizes. (sample observations which are so similar that no additional is gained from all observations following the highest ranked).

Below, we enumerate ways that we believe improve the procedure of evaluating AL strategies with regard to all of the points mentioned:
\paragraph{K.1 Realistic Label Distributions}
The label distribution of a dataset is fixed and AL methods have to be evaluated against them to ensure generalizability. In practice, it cannot be taken for granted that every new dataset has a uniform label distribution. However, the label distribution in combination with the desired properties of the classifier are crucial parameters for selecting the proper training strategy (e.g. weighted loss, upsampling). In addition, query methods might have different interactions with label distributions, for example, explorative and uncertainty-based query methods. 
\textbf{Current Literature} In the current literature, most work is performed on balanced datasets for classification tasks, even though it is seen as a promising direction for AL to have a balanced classifier as the main objective. 
Experiments conducted on artificially imbalanced datasets by \cite{munjalRobustReproducibleActive2022a} with strong SL models show improvements over random.
Similar results were reported by \cite{krishnanImprovingRobustnessEfficiency2021}, but without any adjustments to the training protocol to handle the imbalanced dataset.
Further, \cite{galDeepBayesianActive2017a} undertook experiments on the ISIC-2016 dataset, however, they only included bayesian active learning with a high signal to noise ratio due to the small size of the overall dataset.
Based on these experiments, \cite{atighehchianBayesianActiveLearning2020} benchmarked bayesian active learning on the MIO-TCD dataset showing performance improvements for underrepresented classes.
\textbf{Our Solution} We propose to extend the evaluation of AL for classification to a wider variety of different datasets focusing on different label distributions arising naturally, seeing this as a major use-case for AL methods.
\paragraph{K.2 Realistic Starting Budgets}
When working with a new dataset, the starting budget is either a given or has to be chosen. 
Intuitively one would want to have the smallest starting budget possible to immediately gain performance through AL methods since any further labeling is equivalent to random queries at this point. 
\textbf{Current Literature} Most recent research publications use starting budget sizes with thousands of observations, on datasets s.a. CIFAR-10 and CIFAR-100\cite{munjalRobustReproducibleActive2022a, kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019, mittalPartingIllusionsDeep2019a, yiUsingSelfSupervisedPretext2022}. Information theoretic publications commonly use small starting budgets \cite{galDeepBayesianActive2017a, kirschBatchBALDEfficientDiverse2019a}, but mostly on simple datasets s.a. MNIST \cite{lecunMNISTDatabaseHandwritten1998}, where models already perform reasonable. Some studies with regard to smaller starting budgets mostly in combination with Semi-SL and Self-SL on datasets s.a. CIFAR-10 and CIFAR-100 were performed \cite{bengarReducingLabelEffort2021a,mittalPartingIllusionsDeep2019a,gaoConsistencyBasedSemisupervisedActive2020} often with the conclusion that AL for smaller query sizes does actually hurt performance.
Based on their experiments with multiple initial starting budgets on datasets with different number of classes, \cite{bengarReducingLabelEffort2021a} conclude, that there exist a relationship between number of classes and starting budget.
\textbf{Our Solution} We propose to run AL experiments on multiple different starting budget sizes for each dataset in a systematic manner based on the number of classes a dataset has. This is based on the intuition, that the number of classes can be seen as a proxy for the complexity of the task and is a known parameter before initializing AL.

\paragraph{K.3 Realistic Query Size}
The number of samples queried in one acquisition step is a design choice for an AL method that can not be evaluated in practice. Therefore it has to be clear how to select it for a query method to ensure robustness.
\textbf{Current Literature} In current literature there is a concerning disconnect between theoretical and practical papers regarding to the query size. 
Information theoretical papers typically select the smallest query size possible, as it is deemed a crucial parameter and query methods are designed to simulate smaller query sizes whilst taking bigger ones s.a. BatchBALD \cite{galDeepBayesianActive2017a,kirschBatchBALDEfficientDiverse2019a,pinslerBayesianBatchActive2021}. In contrast, practically oriented papers \cite{kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019a, sinhaVariationalAdversarialActive2019, mittalPartingIllusionsDeep2019a, munjalRobustReproducibleActive2022a} usually select large query sizes. Ablations with regard to the query size were made by \cite{munjalRobustReproducibleActive2022}, concluding that it is not a crucial parameter.  \cite{atighehchianBayesianActiveLearning2020} presented similar results, stating that large query sizes can safely be used. 
In their work \cite{bengarReducingLabelEffort2021a} parse one query size per starting budget without further ablating its importance.
\textbf{Our Solution} We evaluate AL methods with realistic query sizes in relation to the starting budgets and analyze its influence on the performance of the query methods.
\paragraph{K.4 Realistic Method Configuration}
Proper configuration has been shown to be an integral part to obtain a well performing model. 
Since it is the goal of AL to obtain a well performing model with as little labeled data as possible and the model being both used as basis for query and performance measurement, we believe a methodical approach to configuring hyperparameters will lead better comparability across different query methods -- especially if a query method induces a change in training.
\textbf{Current Literature} Most works in AL do not state how hyperparameters for training are obtained \cite{krishnanImprovingRobustnessEfficiency2021, yooLearningLossActive2019, sinhaVariationalAdversarialActive2019, kimTaskAwareVariationalAdversarial2021, mittalPartingIllusionsDeep2019a} -- typically they are identical to the ones used on the whole dataset. In some cases even the query methods are dependent on hyperparameters which are subject to change for different datasets \cite{sinhaVariationalAdversarialActive2019, kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019}.
\cite{munjalRobustReproducibleActive2022a} showed the influence of proper hyperparameter tuning with a validation set by outperforming previous works and ranking of query methods. However, their hyperparameter optimization setup is very costly, as they run a full AutoML hyperparameter selection for every query method and on each training step.
\textbf{Our Solution} We clearly define a validation dataset with a relative size to the initially labeled budget based on which a small set of hyperparameters are selected once for a whole AL pipeline on the initial labeled dataset. These hyperparameters include: learning rate, weight decay and data augmentations \cite{cubukRandaugmentPracticalAutomated2020}  
% (Also maybe Scheduler...).
%  once per label-regime based on a validation set with a comparatively big size. 
The size of the validation set is inspired by \cite{oliverRealisticEvaluationDeep2019}, where they derive based on Hoeffding's inequality \cite{hoeffdingProbabilityInequalitiesSums1994}, that a big validation set is required for model selection.\\
The concept of keeping hyperparameters for multiple different dataset sizes is inspired by \cite{isenseeNnUNetSelfconfiguringMethod2021}, showing that a good set of hyperparameters regularizes well across different datasets with good performance, therefore we argue that this should also be the case for different label settings in AL.
\paragraph{K.5 Realistic Methodological Context}
Recent advances in training strategies, namely Self-Supervised (Self-SL) \cite{chenSimpleFrameworkContrastive2020a, heMomentumContrastUnsupervised2020} and Semi-Supervised Learning (Sem-SL) \cite{sohnFixMatchSimplifyingSemisupervised2020, leePseudolabelSimpleEfficient2013} have shown strong evidence to lower the label effort required for training deep classifiers by making use of large unlabeled datasets (pool).
Since both strategies tackle the same problem as AL and can be combined with each other, we believe that AL strategies should be compared in combination with these strategies.
% This has the possibility to lead to cumulative benefits and use AL in settings which where not applicable beforehand due to poor performance, make better use of representations obtained by Self-SL and stabilize Sem-SL.
\textbf{Current Literature} In their work, \cite{bengarReducingLabelEffort2021a} benchmark Self-SL and SL in combination with AL with the conclusion that the combination of both is not harmful, but AL is only useful after a certain amount of samples are labeled based on classes depending on the training strategy. However, they did not fine-tune their models. \cite{yiUsingSelfSupervisedPretext2022} propose an AL query method using Self-SL pre-training, however, they settle on rotation prediction as pre-training, as it yields a more clearly defined acquisition function, and do not make full use of the power of self-supervised pre-training methods.
Further, \cite{gaoConsistencyBasedSemisupervisedActive2020} combine Semi-SL with AL showcasing superior performance on the datasets where Semi-SL methods were originally proposed and conclude that Semi-SL brings stronger performance gains than pure AL.
Similarly \cite{mittalPartingIllusionsDeep2019} evaluate Semi-SL with AL in standard settings alongside evaluations in the low-label regime. In their setting, Semi-SL again strongly improves the performance of models but does not reliably lead to improvements over random sampling (especially in the low-label regime it can even hurt performance).
\textbf{Our Solution} We propose to compare Self-SL pre-trained, Sem-SL and SL models jointly with the same architecture. 


% Notes:
% \cite{agarwalContextualDiversityActive2020a} use RL based AL with incredible cost for setup of AL but no time at all for hyperparameter optimization!

==> tex/99_depr_tex/02_OLDdepr_relworks.tex <==
% whats special about AL eval? what makes it realistic?
% maybe validation paradox here? (how invasive in intro?)
% and the goals of evaluation
% state that we identified 5 key parameters that define realistic evaluation
% state that we will contrast the current state and related pitfals against our proposed improvement in all 5 topics.
%

%Realistic evaluation in AL is particularly tricky due to a phenomenon we refer to as the \textit{validation paradox}: AL parameters can not be configured on a new data set without directly contradicting the purpose of reducing labeling efforts. Thus, AL application, by definition, implies pre-configured methods to be rolled-out on new data sets. Realistic evaluation needs to reflect these circumstances and test AL methods 1) under a broad range of potential future data and label scenarios and 2) for generalizability of fixed configurations when rolled out on new data sets.

%In this work, we make several improvements over the standard evaluation for deep active classification, which typically follows canonical steps:
%First, a commonly available dataset used for supervised learning is taken and split into an unlabeled pool dataset and small labeled initial dataset.
%As a successive training step, an arbitrary and not necessarily standardized model is then trained on the small labeled dataset. 
%The resulting trained model is then used in conjunction with a query method, to query a fixed amount of samples (defined by the acquisition size) from the pool which are labeled and added to the labeled dataset.
%The performance of the models with specific query methods is then tracked for multiple acquisition steps in a plot with x-axis for labeled samples and y-axis for performance (accuracy etc.).
%Based on this, a recommendation for one query method is then given.
\\
%The choice of datasets, the size of the initial labeled dataset, acquisition size and steps is somewhat standardized across different papers.
%However, why exactly these specific settings with regard to datset, acquisition size or initial labeled budgets are chosen is to our knowledge never fully explained or ablated.
\\
%At least from a theoretical perspective Active Learning is heavily dependent on the above mentioned hyperparameters which are often taken as a given, but potentially vary greatly in practice for new datasets.
%Each acquisition step has a dependency on these values: 1. Training Dataset 2. Final Model (Validation Set and Hyperparameters) 3. Unlabeled Pool 4. Acquisition Size.\\
%If these interact in a specific manner, the \textit{Cold-Start problem} can occur, which is described as (an) AL strategy performing worse than random queries.
%Commonly this phenomenon is observed for small initial datasets and is mostly understood for uncertainty based AL strategies where a `bad model queries useless samples'.
%Therefore having a clear understanding how these interact or how to set up a well generalizing AL strategy with regard to these parameters is crucial.
%This is especially true due to the \textit{validation paradoxon} in AL, meaning that it is not (easily) possible to measure the performance gain (or potential loss) of AL over random queries in a production setting without additional labeling effort (whose reduction the purpose of AL is). 
% \paragraph{Cold-Start Problem} Is commonly attributed when AL strategies perform (much) worse than random sampling (usually at early stages of the AL cycle and small starting budgets). This phenomena is mostly understood for uncertainty based acquisition with high acquisistion sizes. (sample datapoints which are so similar that no additional is gained from all datapoints following the highest ranked).
\\
Below, we enumerate ways that we believe the procedure of evaluating AL strategies could be improved with regard to all of the above mentioned points:
% We aim to investigate the following main question:
% \paragraph{When does Active Learning bring benefits in the context of Deep Classification?} 
% To answer this question, 
\paragraph{Realistic Methodological Context} 
Recent advances in training strategies, namely Self-Supervised \cite{chenSimpleFrameworkContrastive2020a, heMomentumContrastUnsupervised2020} and Semi-Supervised Learning \cite{sohnFixMatchSimplifyingSemisupervised2020, leePseudolabelSimpleEfficient2013} have shown strong evidence to lower the label effort required for training Deep Classifiers.
Since both of these strategies are orthogonal to AL, potentially offering better performing models, and can be combined with each other, we believe that AL strategies should be compared in combination with these strategies.
This has the possibility to lead to cumulative benefits and use AL in settings which where not applicable beforehand due to poor performance, make better use of representations obtained by Self-SL and stabilize Sem-SL.
\subparagraph{Current Literature}
\begin{itemize}
    \item Self-Supervised Learning 
    \begin{itemize}
        \item \cite{bengarReducingLabelEffort2021a} show experiments with Self-SL Pre-Trained Models on CIFAR-10, CIFAR-100 and Tiny ImageNet. In their setting AL only brings benefits for very high label regimes. They hypothesize a correlation between number classes and required labels for AL to beneficial.\\
        We are concerned about bad supervised baseline performance, and wonder how models with good performance have the \emph{Cold-Start Problem}, especially due to small acquisition sizes. 
        \item \cite{yiUsingSelfSupervisedPretext2022} propose an AL query method using Self-SL pre-training however, they settle on rotation prediction as pretraining for a more clearly defined acquisition function and do not make full use of the power of self-supervised Pre-Trained models. Their experiments for classification are performed on CIFAR-10, Caltech-101 and ImageNet-67. Also they show no results for low-label settings.
    \end{itemize}
    \item Semi-Supervised Learning
    \begin{itemize}
        \item \cite{gaoConsistencyBasedSemisupervisedActive2020} combine Semi-Supervised Learning with AL and show results on CIFAR-10, CIFAR-100 and ImageNet. Here they show that Sem-SL can be beneficially for AL and lead to circumventing the cold-start problem in the low label regime, however their supervised baselines are not SOTA using a VGG16 model.
        \item \cite{mittalPartingIllusionsDeep2019} evaluate Semi-Supervised Learning with AL on CIFAR-10 and CIFAR-100 on standard size alongside evaluations in the low-label regime. In their setting Sem-SL again strongly improves the performance of models but does not reliably lead to improvements over random sampling (especially for low-label regime).
    \end{itemize}
\end{itemize}
\subparagraph{Our Solution} We propose to compare Self-SL pre-trained, Sem-SL and SL models jointly with the same architecture. 
\paragraph{Realistic Method Configurations} Proper configuration of models have been shown to be an integral part to obtain a well performing model. 
Since the goal of AL is to obtain a well performing model with as little labeled data as possible, we believe a methodic approach to configuring hyperparameters will lead better comparability across different query methods -- especially if a query method induces a change in training.
\\
% In the current literature about active learning, the importance of this point seems often to be neglected and it is unclear how hyperparameters are selected.
\subparagraph{Current Literature}
\begin{itemize}
    % \begin{itemize}
        \item Many works do not consider stating the way hyperparameters are selected at all and/or select parameters which are commonly used when training on the whole dataset \cite{krishnanImprovingRobustnessEfficiency2021, yooLearningLossActive2019, sinhaVariationalAdversarialActive2019, kimTaskawareVariationalAdversarial2021, mittalPartingIllusionsDeep2019a}.
        \begin{itemize}
            \item Sometimes hyperparameters are even changed for each dataset which are potentially crucial for the acquisition function! \cite{sinhaVariationalAdversarialActive2019} \& potentially \cite{kimTaskAwareVariationalAdversarial2020} (look at \cite{yooLearningLossActive2019})
         \end{itemize}
         \item \cite{munjalRobustReproducibleActive2022a} showed in their paper the influence of proper hyperparameter selection based on Auto-ML for every AL iteration and a validation set using strong regularization and more data augmentation (Randaugment). This setting led to their supervised random baseline performing better and reducing effectiveness of AL strategies.
         \item \cite{mittalPartingIllusionsDeep2019a} made a similar finding using AutoAugment to \cite{munjalRobustReproducibleActive2022a} (CIFAR-10, CIFAR-100).
    % \end{itemize}
\end{itemize}
\subparagraph{Our Solution} Clearly define a validation dataset with a relative size to the initially labeled budget based on which a small set of hyperparameters are selected once for a whole AL pipeline on the initial labeled dataset.
These hyperparameters are: Learning Rate, Weight Decay and DataAugmentations (RandAugment)  (Also maybe Scheduler...).
%  once per label-regime based on a validation set with a comparatively big size. 
The size of the validation set is inspired by \cite{oliverRealisticEvaluationDeep2019}, where they derive that a big validation set is needed for model selection based on Hoeffding's inequality (cite).\\
As has been shown by \cite{isenseeNnUNetSelfconfiguringMethod2021} a good set of hyperparameters regularizes well across different datasets with good performance, therefore we argue that this should also be the case for different label settings in AL.
% Further we allow some knowledge to flow across datasets, as a bias from which hyperparameters are selected.
% TODO: -> RESULTS/Conclusion...
% This approach to hyperparameter selection gives a general guideline and reduces hyperparameter selection cost compared to \cite{munjalRobustReproducibleActive2022a}, while leading to comparable performance for our supervised models. 
% This allows for fast transfer of AL settings to new datasets.
\paragraph{Realistic Data Scenarios}
AL, if used in practice, will need to generalize well across different datasets by performing better than random queries or have extremely clear guidelines showcasing how to set it up.
This is because differently to Sem-SL and Self-SL it is not possible to validate the performance gain (or even potential loss) obtained by AL through comparisons in practice since this can only be evaluated if the whole dataset is labeled.
% -- which is exactly what one wants to avoid to do if performing AL.
Therefore we deem it crucial, that AL methods are evaluated in different settings to showcase their robustness against them and/or validate that the proposed set up works reliably.\\ 
% Most research is asking the question what AL strategy performs best and there is no consensus on which works best.\\
% We believe it is most crucial to know in which setting AL systematically outperforms random and/or how AL has to be formulated and set up, that it reliably performs better than random.

% TODO: Restructure this!
\subparagraph{Current Literature}
%%%%%%%%% OLD VERSION %%%%%%%%%%%%
% \begin{itemize}
    % \item Information Theoretic Papers:
    % \begin{enumerate}
    %     \item Small initial labeled budget, small acquisition size \cite{galDeepBayesianActive2017a,kirschBatchBALDEfficientDiverse2019a}
    %     \item Not much work showcasing applicability to real-world problems with good performance (too many trainings on realistic problems)
    % \end{enumerate}
    % \item Validation Paradoxon, reliably better than/as good as random
    % \begin{itemize}
    %     \item \cite{bengarReducingLabelEffort2021a} use both Self-SL and Supervised models on three datasets (CIFAR-10, CIFAR-100 and Tiny ImagenNet) for multiple data regimes.
    %     \item \cite{mittalPartingIllusionsDeep2019} use both Sem-SL and Supervised models in the low data regime to asses the performance of AL in these settings.
    %     \item In production environments we are not solely interested in the \% of labeled data and the relative performance, but mostly in the amount of labels required to solve a task succesfully.
    % \end{itemize}
    % \item Cold-Start Problem -- AL performs worse than random (initial budget \& Aquisition Size)
    % \begin{itemize}
    %     \item The Cold-Start Problem, which is commonly attributed to a bad performing classifier with Uncertainty based AL in early stages of AL iterations which is especially problematic combination with acquisition sizes greater than one sample \cite{gaoConsistencyBasedSemisupervisedActive2020}.
    %     \item How do explorative strategies work?
    % \end{itemize}
    % \item Imbalanced Datasets -- In practice for AL pipelines need to be robust regardless of the distribution of ground truth samples. There
    % \begin{itemize}
    %     \item \cite{munjalRobustReproducibleActive2022a} evaluate the performance of AL on the artificially imbalanced CIFAR-10 LT dataset with strong baselines. 
    %     % TODO: Add proceedings version of Krishnan et al.
    %     \item \cite{krishnanImprovingRobustnessEfficiency2021} evaluate the performance of AL on CIFAR-10 LT.
    %     \item Experiments on these artificially created datasets have to be taken carefully and are highly dependent on the exact creation of imbalance.
    %     \item \cite{atighehchianBayesianActiveLearning2020} perform experiments with Bayesian Active Learning on Mio-TCD showing an performance increase for underrepresented classes.
    %     \item \cite{galDeepBayesianActive2017a} perform experiments on ISIC-2019 only using Bayesian Active Learning.
    %     \item No experiments with Self-SL and Sem-SL in combination with AL on 
    % \end{itemize}
    % \item Dependence on Pool, but AL has to generalize (Unkown, Acquisition Size, Initial Budget, Variety of Datasets)
    % \begin{itemize}
    %     \item Currently most AL research for Classification is focused on the datasets CIFAR-10, CIFAR-100, Tiny ImageNet. 
    %     \item Using a subset of the pool for their acquisition function \cite{atighehchianBayesianActiveLearning2020} (add more citations), and claiming either performance benefits or neglegible loss in performance while speeding up. 
    %         We wonder about this, since AL in theory should be most powerful if it can select samples from a big pool (choice only meaningful if there is enough to choose from).
    %     \item Most practical AL is evaluated in the same label regimes which is 1000 to 10000 samples or 5000 to 20000 samples. To our knowledge there is no reason behind this.
    %     \item For many real world tasks when a dataset is started to be created an initial amount of labeled data in this quantity can correspond to the whole budget for labeling.
    %     \item In research one often just wants one well performing model on a dataset and creates a dataset just for this -- try to reduce labelling effort as much as possible.
    % \end{itemize}
    % \item Acquisition Size -- There is no conses about importance of the value of acquisition size. 
    % \begin{itemize}
    %     % TODO: Add paper with MMD BatchMI and some other theoretical works
    %     \item More theoretical papers \cite{galDeepBayesianActive2017a,kirschStochasticBatchAcquisition2022,kirschBatchBALDEfficientDiverse2019} usually use very small initial label budgets and small acquisition sizes.
    %     Even going so far as to derive new acquisition functions to allow acquiring more samples in one AL step, making it in theory on of the most crucial parameters to fully unleash the power of AL.
    %     % Question: There could stand a very long list for both of these points... Do we want this?
    %     \item This stands in contrast to the big acquisition sizes used in papers which are more practically inclined \cite{sinhaVariationalAdversarialActive2019,bengarReducingLabelEffort2021a,yooLearningLossActive2019,mittalPartingIllusionsDeep2019}.
    %     \item \cite{munjalRobustReproducibleActive2022a} made an ablation study on the parameter of acquisition size with supervised models and concluded that this parameter did not change their results in a meaningul manner.
    %     \item We deem this strong disconnect between theoretical works and practical works on AL as highly problematic and aim to investigate this. One clear difference is the amount of initially labeled data and the relative pool size.
    % \end{itemize}
% \end{itemize}
\begin{itemize}
    \item Initial Budget
    \begin{itemize}
        \item Information Theoretic Papers use AL with smallest initial label budget sizes possible (on anything more complex than NIST datasets this proves complicated due to bad performance)
        \item Practical oriented Papers use AL usually with initial label budget sizes with 1k to 5k samples 
    \end{itemize}
    \item Acquisition Size
    \begin{itemize}
        \item Information Theoretic Papers use AL with smallest feasible acquisition size possible (to high acquisition sizes hurt performance) and propose query functions to allow bigger acq. sizes (e.g. BatchBALD)
        \item Practical oriented papers use AL with big acquisition sizes 1k-5k samples (ablation exist that acq. size is no crucial parameter)
    \end{itemize}
    \item Literature in right direction:
    \begin{itemize}
        \item \cite{bengarReducingLabelEffort2021a} use both Self-SL and Supervised models on three datasets (CIFAR-10, CIFAR-100 and Tiny ImagenNet) for multiple data regimes. -- AL has trouble on Self-SL
        \item \cite{mittalPartingIllusionsDeep2019} use both Sem-SL and Supervised models in the low data regime to asses the performance of AL in these settings.
        \item \cite{munjalRobustReproducibleActive2022a} made an ablation study on the parameter of acquisition size with supervised models and concluded that this parameter did not change their results in a meaningul manner.
        \item \cite{gaoConsistencyBasedSemisupervisedActive2020} made an ablation study for low data on ... and found that AL performed in fact worse than random acquisition
    \end{itemize}
    \item Cold Start -- can be possibly left out
    \begin{itemize}
        \item is mostly understood as a bad performing classifier with Uncertainty based AL in early stages of AL iterations which is especially problematic combination with acquisition sizes greater than one sample \cite{gaoConsistencyBasedSemisupervisedActive2020}
        \item this direction is similar to \cite{kirschBatchBALDEfficientDiverse2019a} where they propose a new Query Method which avoids querying too many similar samples.
    \end{itemize}
    \item Label Distribution represents a dataset inherent parameter which is not generally known beforehand but plays an important role
    \begin{itemize}
         \item \cite{munjalRobustReproducibleActive2022a} evaluate the performance of AL on the artificially imbalanced CIFAR-10 LT dataset with strong baselines. 
         \item \cite{krishnanImprovingRobustnessEfficiency2021} evaluate the performance of AL on CIFAR-10 LT with a different imbalance factor.
         \item \cite{atighehchianBayesianActiveLearning2020} perform experiments with Bayesian Active Learning on Mio-TCD showing a performance increase for underrepresented classes.
         \item \cite{galDeepBayesianActive2017a} perform experiments on ISIC-2019 only using Bayesian Active Learning.
    \end{itemize}
\end{itemize}
\subparagraph{Our Solution} Benchmark performance of AL strategies on multiple different datasets (CIFAR-10, CIFAR-10-LT, CIFAR-100, ISIC-2019, MIO-TCD) for three different labeling settings with different acquisition sizes and initial budgets.
We select these label regimes to be dependent upon the number of classes based on the intuition, that the number of classes can be seen as a proxy for the `hardness' of the classification task.
Also we believe it safe to assume that this parameter should be known when performing AL.
% since this is a parameter that we believe should be known in all cases when performing AL.
This setup allows to evaluate the influence of the initial labeled set, validation set and acquisition size on the performance of AL strategies by using overlapping label regions.

% TODO: where to put this?
% \cite{munjalRobustReproducibleActive2022a} note that even AL outperforming random in a statistically relevant way is not always a given, even on the datasets and label settings many AL strategies were formulated and proposed.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% old version %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Improved Evaluation}
% % Reformulate the following based on a Realistic Evaluation of Sem-SL:
% In this work, we make several improvements to the conventional experimental procedures used to evaluate Active Learning methods,
% which typically proceeds as follows: First, take a common (typically image classification) dataset used for supervised learning 
% and throw away the labels for most of the dataset. 
% Then, treat the portion of the dataset whose labels were retained as a small labeled dataset $\mathcal{D}$ and the remainder as an 
% the remainder as an unlabeled Pool $\mathcal{D}_{}$. Some (not necessarily standard) model is then trained 
% and accuracy is reported using the unmodified test set. The choice of dataset and number of retained labels is 
% somewhat standardized across different paper (, however, these are purely based on heuristics).\\
% % 
% The answer they want to give is which Active Learning strategy (Query Function) should you use in your experiments.
% Since this is only based on the performance of the final model, we believe that this recipe could use some updates.
% Active Learning is dependent on the following parameters: 1. Training Set, 2. Model, 3. Validation Set, 4. Distribution of the Pool. 
% All of these can vary greatly and according to different papers do or do not have a significant effect on the effect of AL.
% However, the first question we should ask is: should you use Active Learning in general for your specific setting.\\
% \\
% Below, we enumerate ways that we believe this procedure can be made more applicable to real-world settings.

% \paragraph{Comparing Self-Supervised, Semi-Supervised and Supervised Learning}
% Self-Supervised and Semi-Supervised Learning both work on remarkably similar settings to Pool based Active Learning and both of them claim to offer a great reduction of labeling effort to train good performing models.\\
% In this context we argue that the incorporation of these techniques into the AL setup is only a logical step with the potential of cumulative benefits.
% \paragraph{Comparing Performance across multiple different `Label Regimes'.}
% By using different label regimes with overlaps we believe it is possible to observe the effect of multiple parameters at once.\\
% These are for the setting we built: 1. Initial Dataset Size 2. Acquisition Size 3. Validation Dataset Size\\
% By reviewing model performance at a certain number of labeled samples with different starting points and acquisition sizes it is possible to observe the importance of these parameters.\\
% \subparagraph*{Using Validation Datasets}
% By having a systematic approach of using a validation set, we can employ the act of hyperparameter tuning and model selection based on validation performance. Both of which have a great impact on model performance and in some cases allow to increase the performance by proper hyper-parameter selection to that of models using 5x the amount of data.
% \paragraph{Considering Class Distribution Mismatch \& `Label Noise/Data Cleanliness'}
% Active Learning
% By considering class distribution mismatches with multiple different datasets and 

==> tex/99_depr_tex/02_relworks_paul.tex <==


\subsection{AL Task Formulation}\label{ss:task-formulation}
As depicted in \cref{fig:main-concept}, AL describes a classification task, where a dataset $\mathcal{D}$ is given that is divided into a labeled set $\mathcal{L}$ and an unlabeled pool $\mathcal{U}$. Initially, only a fraction of the data is labelled ("starting budget"), which is ideally split further into a training set and a validation set for hyperparameter (HP) tuning and performance monitoring. After initial training, the QM is used to generate queries $\mathcal{Q_U}$ of a certain amount ("query size") that represent the most informative samples from $\mathcal{U}$ based on the current classifier predictions. Subsequently, queried samples are labeled ($\mathcal{Q_L}$), moved from $\mathcal{U}$ to $\mathcal{L}$, and the classifier is re-trained on $\mathcal{L}$. This process is repeated until classifier performance is satisfying, as monitored on the validation set. 
%\\
%From a more abstract perspective, the goal of AL is to use the information of the labeled dataset $\mathcal{L}$ and the prediction function $f_\theta(x)$, to find the observations giving the most information where $p(y|x)$ deviates from $f_\theta(x)$. 
%  Active Learning is a game of reducing cost -- one trades in computation cost with the expectation of lowering labeling cost which is deemed to be the bottleneck.
%This is also being reflected by the way performance in AL is measured -- which is the relative performance gain of the prediction function with queries from a QM compare to random queries.
%Making the prediction function implicitly the gauge for measuring the "success" of an AL strategy.
%\\
%A comprehensive overview over AL and its methods is out of the scope of this paper, we refer interested readers to \cite{}. 
%Instead, we focus on the class of QM which solely use the prediction function as a basis for their queries, and otherwise leave the training-strategy and model unchanged.
%In addition, methods belonging to this category currently hold the state-of-the-art in AL on classification tasks, while also being operational less complex to implement. 
%Further, they require no additional hyperparameters to be set for the query function which is hard to evaluate in practice due to the validation paradoxon.
%\\
%Overall, the methods we consider fall into two classes: explorative strategies, which enforce queried observations to explore the distribution of $p(x)$; and uncertainty based strategies, which make direct use of the prediction function $f_\theta(x)$.
%\footnote{This is conceptually similar to the exploration and exploitation paradigm seen in Reinforcement Learning and there actually exist strong parallels between Reinforcement Learning and Active Learning -- so much so that Reinforcement Learning has been proposed to use in AL and AL based strategies have been proposed to be used in Reinforcement Learning.}
%The principled combination of both strategies, especially to allow higher query sizes for uncertainty based QM, is an open research question.
%\\
\subsection{What is special about evaluation in Active Learning?}\label{ss:realistic-eval}
Evaluating an AL algorithm typically means testing how much classification performance is gained by data samples queried and added over several training iterations. The QM selecting those samples is considered useful if the performance gains exceed the gains of randomly queried samples. While this process is well-established, it is prone to over-simplification of how AL algorithms are applied in practice and thus neglecting critical concepts for realistic evaluation. 

\noindent \textbf{AL validation paradox} Upon application, AL parameters can not be adapted to the dataset at hand. This is because validating the choice of a QM or query size, for instance, implies several parallel query/label trajectories, which directly contradicts AL's purpose of reducing labeling efforts. Thus, AL application, by definition, implies rolling out pre-configured AL settings on a new dataset. Realistic evaluation needs to reflect these circumstances by 1) identifying generalizing AL settings and 2) testing the generalizability of fixed settings when rolled out on new datasets. Identifying such settings requires evaluating QMs under a broad range of potential future data and label scenarios including various datasets, starting budgets, label distributions, and query sizes. This search space can be reduced if a method is developed for a specific application including e.g. a pre-defined data domain or starting budget size.

\noindent \textbf{Cold start problem} If generalizability is not tested for, the QM might fail in practice, because external factors such as limited compute or labeling budgets may lead to deviations of AL parameters from the evaluation setting. Such failure of QMs, i.e. sub-random performance, is a known issue in the research community and commonly referred to as the \textit{cold start problem} (\cite{gaoConsistencyBasedSemisupervisedActive2020}).  

\noindent \textbf{Adequate baselines} Another critical aspect of AL evaluation is the fact that a well-performing classifier is the final goal of any AL method. This goal implies a strong interconnection of AL performance with other classifier parameters. For instance, a QM should not be considered useful as long as the same performance gains can be obtained by simple modifications of the learning rate, data augmentation, or by employing alternative training paradigms such as Self-SL or Semi-SL. Thus, QMs need to be evaluated on well-configured classifiers and compared against or combined with other competitive training paradigms. 

%1) Realistic spectrum of parameters needs to be checked across various datasets. Potential outcomes: QM is agnostic and works on the entire spectrum, or identify area where QM works on various datasets. Output: fixed setting to be applied in practice. Shortcut: Special task interest (small starting budget, small query size) can naturally limit the search space. Importantly the "QM works" statement is also conditioned on the certain K4 K5 setting, which should also be optimized.
%2) Only K4 K5 can be adapted on the starting budget of the new dataset, the rest needs to be rolled-out as is.
%
%
\subsection{Current pitfalls of AL evaluation}\label{ss:eval-protocol}

The current AL literature features an inconsistent landscape of evaluation protocols, but none of them adhere to the concepts for realistic evaluation described above (see \cref{tab:relworks} and \cref{s:app-relworks}). To make these general concepts more concrete, we identify five key \textit{pitfalls} (P1-P5) that need to be overcome for meaningful evaluation of QMs. For an overview of the pitfalls and how they integrate into the AL setting see \cref{fig:main-concept}. 

%K1: Data distribution. Teilaspekte: Class distribution. Class complexity. Mismatch class importance versus frequency
%K2: Starting budget. Pitfall: AL used to late or too early (cold start).
%K3: Too small (too much compute) or too large (less AL effect / iteration, prone to cold start)
%
\textbf{P1: Lack of evaluated data distribution settings}
To ensure that QMs work out-of-the-box in real-life settings, they need to be evaluated on a broad data distribution. Relevant aspects of a distribution in the AL-context go beyond the data domain and include class distribution, the relative difficulty of separation across classes, as well as a potential mismatch between the frequency and importance of classes. All of these aspects directly affect the functionality of a QM and may lead to real-life failure of AL when not considered in the evaluation.
\textbf{Current practice:} Most current work is limited to evaluating QMs on balanced datasets from one specific domain (e.g. CIFAR-10/100) and under the assumption of equal class importance. To our knowledge, testing the generalizability of a fixed QM setting to new datasets ("roll-out") has not been performed before. There are some experiments conducted on an artificially imbalanced dataset (CIFAR-LT)  \cite{munjalRobustReproducibleActive2022a,krishnanImprovingRobustnessEfficiency2021} suggesting good AL performance. Further, \citet{galDeepBayesianActive2017a} studied AL on the ISIC-2016 dataset, but obtained volatile results due to the small dataset size. \citet{atighehchianBayesianActiveLearning2020} studied AL on the MIO-TCD dataset and reported performance improvements for underrepresented classes.
In the large study \citet{beckEffectiveEvaluationDeep2021} perform experiments on five datasets out of which three are toy datasets and \cite{zhanComparativeSurveyDeep2022a} perform experiments on 13 datasets out of which four datasets are toy datasets.
\textbf{Proposed solution:} We argue that the underrepresentation of class-imbalanced datasets in the field is one reason for current doubts regarding the general functionality of AL. Real-life settings will most likely not be class balanced providing a natural advantage of AL over random sampling. We propose to consider diverse datasets with real class imbalances as an essential part of AL evaluation and advocate for the inclusion of "roll-out" datasets, as a real-life test of selected and fixed AL settings.

%
%
\textbf{P2: Lack of evaluated starting budget}
There are two reasons for why this parameter is an essential aspect of AL evaluation: 1) Upon application, the budget might be fixed and the QM is required to generalize out-of-the-box to this setting. 2) We are interested in the minimal budget at which the QM works since a too large budget implies inefficient labeling (equivalent to random queries) and a too small budget is likely to cause AL failure (cold start problem). This search needs to be performed prior to an AL application due to the validation paradox. 
\textbf{Current practice:} Most recent studies evaluate AL on a single starting budget made of thousands of samples on datasets such as CIFAR-10 and CIFAR-100\cite{munjalRobustReproducibleActive2022a, kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019a, yiUsingSelfSupervisedPretext2022}. Information-theoretic publications commonly use a smaller starting budget \cite{galDeepBayesianActive2017a, kirschBatchBALDEfficientDiverse2019a}, but typically on even simpler datasets such as MNIST \cite{lecunMNISTDatabaseHandwritten1998}. 
\citet{beckEffectiveEvaluationDeep2021} compared two starting budgets on MNIST reporting no performance drop.
On the other hand, some studies benchmarking AL against Semi-SL and Self-SL compare two \cite{bengarReducingLabelEffort2021a} or three \cite{mittalPartingIllusionsDeep2019,gaoConsistencyBasedSemisupervisedActive2020} starting budgets  often with the conclusion that smaller starting budgets lead to AL failure. 
\citet{bengarReducingLabelEffort2021a} reported that there exists a relationship between the number of classes in a task and the optimal starting budget (the intuition being that class number is a proxy for task complexity).
\textbf{Proposed solution:} To overcome this pitfall and resolve the current contradictions, we evaluate all QMs for three different starting budgets on all datasets (low-, mid-, and high-label regimes). Extending on the findings of \cite{bengarReducingLabelEffort2021a}, adequate budget sizes are determined using heuristics based on the number of classes per task. 

%
%
\textbf{P3: Lack of evaluated query sizes}
The number of samples queried for annotation per acquisition step is essential to a realistic evaluation of QMs. This is because, upon application, this parameter might be predefined by the compute-versus-label cost ratio of the respective task (a smaller query size amounts to more compute but might enable more informed queries and thus less labeling). Since query size cannot be validated on the task at hand due to the validation paradox, the generalizability of QMs to various settings of this parameter needs to be evaluated beforehand.
\textbf{Current practice:} In current literature, there is a concerning disconnect between theoretical and practical papers regarding what constitutes a reasonable query size. 
Information-theoretical papers typically select the smallest query size possible and QMs such as BatchBALD are specifically designed to simulate reduced query sizes \cite{galDeepBayesianActive2017a,kirschBatchBALDEfficientDiverse2019a,pinslerBayesianBatchActive2021}. In contrast, practically-oriented papers usually select larger query sizes \cite{kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019a, sinhaVariationalAdversarialActive2019a, mittalPartingIllusionsDeep2019, munjalRobustReproducibleActive2022a}, but only in combination with large starting budgets (P2), where cold start problems generally do not occur. Only a few studies perform limited evaluations of varying query sizes. 
\citet{beckEffectiveEvaluationDeep2021,zhanComparativeSurveyDeep2022a} reporting a negligible effect of varying query sizes, but only tested in combination with large starting budgets (1000 samples). In line with this, \citet{munjalRobustReproducibleActive2022a} conclude that the choice of query size does not matter, but only compared two large values (2500 versus 5000 samples) on a fixed large starting budget (5000 samples). \citet{atighehchianBayesianActiveLearning2020} come to a similar conclusion, but only considered a relatively large starting budget (500) for ImageNet-pretrained models on CIFAR-10, where, again, no cold start problem occurs. \citet{bengarReducingLabelEffort2021a} employ varying query sizes without further analysis of the parameter.
\textbf{Proposed solution:} To overcome this pitfall and reliably study the effect of query sizes also in low-label, i.e. high-risk, settings, we evaluate all QMs for three different query sizes in combination with varying starting budgets on all datasets. 
For a specific focus on the effect of query size in the low-label settings, we perform an additional ablation with varying query sizes on a small fixed starting budget.

%K4 goal: valid comparison. 
%
\textbf{P4: Neglection of the classifier configuration}
As stated in \cref{ss:realistic-eval}, when aiming to draw conclusions about the performance or usefulness of a QM, it is critical that this evaluation be based on well-configured classifiers. Otherwise, performance gains might be attributed to AL that could have been achieved by simple HP modifications. Separating a validation split from the training data is a crucial requirement for sound HP tuning.
\textbf{Current practice:} Most studies in AL literature do not report how HPs are obtained and do not mention the use of validation splits \cite{krishnanImprovingRobustnessEfficiency2021, yooLearningLossActive2019a, sinhaVariationalAdversarialActive2019a, kimTaskAwareVariationalAdversarial2021, mittalPartingIllusionsDeep2019}. Typically, reported settings are copied from fully labeled data scenarios. In some cases, even proposed QMs themselves feature delicate HPs without reporting how they were optimized raising the question of whether these settings generalize on new data \cite{sinhaVariationalAdversarialActive2019a, kimTaskAwareVariationalAdversarial2021, yooLearningLossActive2019a}.
\citet{munjalRobustReproducibleActive2022a} demonstrate how adequate HP tuning on a validation set allows a random query baseline to outperform current QMs under their originally proposed HP settings. However, they run a full grid search for every QM and AL training iteration, which might not be feasible in practice.
\textbf{Proposed solution:} To overcome this pitfall and enable meaningful performance assessment of AL methods, we define a validation dataset of a size deducted heuristically from the starting budget. Based on this data, a small selection of HPs (learning rate, weight decay and data augmentations \cite{cubukRandaugmentPracticalAutomated2020}) is tuned only once per AL experiment while training on the starting budget. The limited search space and discarding of multiple tuning iterations result in a lightweight and practically feasible protocol for classifier configuration.
%
%The size of the validation set is inspired by \cite{oliverRealisticEvaluationDeep2019}, where they derive based on Hoeffding's inequality \cite{hoeffdingProbabilityInequalitiesSums1994}, that a sufficiently large validation set is required for model selection.\\
%The concept of keeping hyperparameters for multiple different dataset sizes is inspired by \cite{isenseeNnUNetSelfconfiguringMethod2021}, showing that a good set of hyperparameters regularizes well across different datasets with good performance, therefore we argue that this should also be the case for different label settings in AL.
%

%
\textbf{P5: Neglection of alternative training paradigms}
Analogously to arguments made in P4, meaningful evaluation of AL requires comparison against alternative approaches that address the same problem. Specifically, the training paradigms Self-SL \cite{chenSimpleFrameworkContrastive2020a, heMomentumContrastUnsupervised2020} and Semi-SL \cite{sohnFixMatchSimplifyingSemisupervised2020, leePseudolabelSimpleEfficient2013} have shown strong potential to make efficient use of an unlabeled data pool in a classification task thus alleviating the labeling burden. Additionally to benchmarking AL against Self-SL and Semi-SL, the question arises of whether AL can yield performance gains when combined with these paradigms.
\textbf{Current practice:} While most AL studies do not consider Self-SL and Semi-SL, there are a few recent exceptions: \citet{bengarReducingLabelEffort2021a} benchmark AL in combination with Self-SL and conclude that AL only yields gains under sufficiently high starting budgets. However, these results were obtained without adequate classifier configuration (P4). \citet{yiUsingSelfSupervisedPretext2022} propose a QM in combination with Self-SL, but only leverage the fraction of Self-SL potential compatible with the proposed QM. Further, \citet{gaoConsistencyBasedSemisupervisedActive2020} combine Semi-SL with AL and report superior performance compared to ST for CIFAR-10/100 and ImageNet \cite{russakovskyImageNetLargeScale2015a}, i.e. the datasets on which Semi-SL methods have been developed. Similarly, \citet{mittalPartingIllusionsDeep2019} evaluate the combination of Semi-SL and AL on CIFAR-10/100, reporting strong improvements compared to standard AL training and find that AL decreases performance for small starting budgets.
\textbf{Proposed solution:} To overcome this pitfall and resolve current inconsistencies, we benchmark all QMs against  both Self-SL and Semi-SL, and evaluate the combination of AL with these paradigms. Crucially, we are the first to study these relations in a trustworthy setting, i.e. while avoiding all other key pitfalls of realistic AL evaluation (P1-P4).


% Exact Recipes: how to work against validation paradox + K4K5
% default: test all the spectra: possible results agnosticity or only one fixed setting
% Exception: special task interest, limit spectrum
% could also guess fixed setting but not recomended way
% K4 K5 can be tuned on the dataset upon applicaiton. Pitfall: statement "QM works" conditioned (K4, K5). Change K4, K5 can lead to drops on new dataset because statement under new condition not been tested.
% K4 K5 important because statement is conditioned on them.
% How do we deal with K4 K5 interacting with QM? Not at all. -> Blindflug
% QM auf neuem dataset does not work. consequence of evaluation not according to our recipe. "aktiv entgegenwirken" - >K1-K3 wegen generalisierung, als K4K5 anpassen auf neues dataset. 
% Story K3: first did not test the spectrum (only fixed ratio starting budget zu K3. common practice get K3 from K2), We saw this was not good enough! Ran extra tests on smaller K3, saw BALD gets more robust.
% Batch Bald simuliert kleinere K3, "Batch Bald works" = "Bald works on small K3".

%



%\subsection{Self-Supervised (Learning) Pre-Training}\label{sec:03-selfsl}
%The high-level concept of Self-SL pre-training is to obtain a model by training it with a proxy task which is not dependent on annotations leading to representations that generalize well to a specific task.
%This allows to induce information from unlabeled data into the model in form of an initialization which can be interpreted as a form of bias.
%Usually these representations are supposed to be clustered based on some form of similarity which is often induced directly by the proxy task and also the reason why different proxy tasks are useful for different downstream tasks.
%Several different Self-SL pre-training strategies were developed based on different tasks s.a. generative models or clustering \cite{}, with contrastive training being currently the de facto standard in image classification.

%\subsection{Semi-Supervised Learning}\label{sec:03-semisl}
%In Semi-SL the core idea is to regularize $f_\theta(x)$ by inducing information about the structure of $p(x)$ of the unlabeled pool in combination with the labeled dataset.
%Usually this leads to the representations of unlabeled observations being more clustered according to the prediction structure of the supervised task.
%Several different Semi-SL methods were developed based on regularizations on unlabeled observations which often fall into the category of enforcing consistency of predictions against perturbations and/or reducing the uncertainty of predictions \cite{}. 
%\footnote{It is also a fair argument that Self-SL pre-trained models is also a form of Semi-SL if finetuned on a small labeled subset.}



% Notes:
% \cite{agarwalContextualDiversityActive2020a} use RL based AL with incredible cost for setup of AL but no time at all for hyperparameter optimization!


% In this work, we make several improvements over the standard evaluation for deep active classification, which typically follows defined canonical steps:
%First, a commonly available dataset used for supervised learning is split into an unlabeled pool dataset and small labeled initial dataset. As a successive training step, an arbitrary and not necessarily standardized model is then fitted on the small labeled dataset. The resulting trained model is then employed in conjunction with a QM to select a fixed amount of samples (defined by the query size) from the pool, which are labeled and added to the labeled dataset as an acquisition step. Finally, the performance of the model and QM pair is tracked over multiple acquisition steps, successively increasing the query size. Based on the results, a recommendation with regard to which QM is `best' then given.

%The choice of dataset, initial small labeled dataset size, and acquisition steps are to a large extend standardized across different papers. However, to our knowledge, it is never fully explained or ablated \textbf{\emph{why}} exactly these standardized settings are chosen. In theory, AL heavily dependents on these settings, which are often considered to be given but potentially vary greatly in practice for new datasets and different sampling strategies.\\ 



%Further, the acquisition step itself depends on the training dataset, final model (which per se depends on the validation set and hyperparameters), unlabeled pool and query size. If these dependencies interact in an unfortunate manner, the \textit{Cold-Start problem} can occur, the event when an AL strategy performs worse than random queries. Commonly this phenomenon is observed on small initial datasets and for uncertainty based AL strategies understood as the situation where a ``bad model queries useless samples''. Therefore having a clear understanding of how the dependencies of the acquisition step interact and how to set up a well generalizing AL strateg is crucial for a successful application of AL.\\

%The importance of these factors is further emphasized by taking into account the \textit{validation paradoxon}, stating that in a model-employed setting it is not without large difficulty to measure the change in performance through AL compared to random queries without including large additional labeling effort (whose reduction the purpose of AL is).\\
% \paragraph{Cold-Start Problem} Is commonly attributed when AL strategies perform (much) worse than random sampling (usually at early stages of the AL cycle and small starting budgets). This phenomena is mostly understood for uncertainty based acquisition with high acquisistion sizes. (sample observations which are so similar that no additional is gained from all observations following the highest ranked).


==> tex/99_depr_tex/02_relworks_update.tex <==
\subsection{AL Task Formulation}\label{ss:task-formulation}
As depicted in \cref{fig:main-concept}, AL describes a classification task, where a dataset $\mathcal{D}$ is given that is divided into a labeled set $\mathcal{L}$ and an unlabeled pool $\mathcal{U}$. Initially, only a fraction of the data is labelled ("starting budget"), which is ideally split further into a training set and a validation set for hyperparameter (HP) tuning and performance monitoring. After initial training, the QM is used to generate queries $\mathcal{Q_U}$ of a certain amount ("query size") that represent the most informative samples from $\mathcal{U}$ based on the current classifier predictions. Subsequently, queried samples are labeled ($\mathcal{Q_L}$), moved from $\mathcal{U}$ to $\mathcal{L}$, and the classifier is re-trained on $\mathcal{L}$. This process is repeated until classifier performance is satisfying, as monitored on the validation set. 


\subsection{What is special about evaluation in Active Learning?}\label{ss:realistic-eval}
Evaluating an AL algorithm typically means testing how much classification performance is gained by data samples queried and added over several training iterations. The QM selecting those samples is considered useful if the performance gains exceed the gains of randomly queried samples. While this process is well-established, it is prone to over-simplification of how AL algorithms are applied in practice and thus neglecting critical concepts for realistic evaluation. 

\noindent \textbf{AL validation paradox} Upon application, AL parameters can not be adapted to the dataset at hand. This is because validating the choice of a QM or query size, for instance, implies several parallel query/label trajectories, which directly contradicts AL's purpose of reducing labeling efforts. Thus, AL application, by definition, implies rolling out pre-configured AL settings on a new dataset. Realistic evaluation needs to reflect these circumstances by 1) identifying generalizing AL settings and 2) testing the generalizability of fixed settings when rolled out on new datasets. Identifying such settings requires evaluating QMs under a broad range of potential future data and label scenarios including various datasets, starting budgets, label distributions, and query sizes. This search space can be reduced if a method is developed for a specific application including e.g. a pre-defined data domain or starting budget size.

\noindent \textbf{Cold start problem} If generalizability is not tested for, the QM might fail in practice, because external factors such as limited compute or labeling budgets may lead to deviations of AL parameters from the evaluation setting. Such failure of QMs, i.e. sub-random performance, is a known issue in the research community and commonly referred to as the \textit{cold start problem} (\cite{gaoConsistencyBasedSemisupervisedActive2020}).  

\noindent \textbf{Adequate baselines} Another critical aspect of AL evaluation is the fact that a well-performing classifier is the final goal of any AL method. This goal implies a strong interconnection of AL performance with other classifier parameters. For instance, a QM should not be considered useful as long as the same performance gains can be obtained by simple modifications of the learning rate, data augmentation, or by employing alternative training paradigms such as Self-SL or Semi-SL. Thus, QMs need to be evaluated on well-configured classifiers and compared against or combined with other competitive training paradigms. 


\subsection{Current pitfalls of AL evaluation}\label{ss:eval-protocol}

The current AL literature features an inconsistent landscape of evaluation protocols, but none of them adhere to the concepts for realistic evaluation described above (see \cref{tab:relworks} and \cref{s:app-relworks}). To make these general concepts more concrete, we identify five key \textit{pitfalls} (P1-P5) that need to be overcome for meaningful evaluation of QMs. For an overview of the pitfalls and how they integrate into the AL setting see \cref{fig:main-concept}. 


\textbf{P1: Lack of evaluated data distribution settings}
To ensure that QMs work out-of-the-box in real-life settings, they need to be evaluated on a broad data distribution. Relevant aspects of a distribution in the AL-context go beyond the data domain and include class distribution, the relative difficulty of separation across classes, as well as a potential mismatch between the frequency and importance of classes. All of these aspects directly affect the functionality of a QM and may lead to real-life failure of AL when not considered in the evaluation.


%
%
\textbf{P2: Lack of evaluated starting budget}
There are two reasons why this parameter is an essential aspect of AL evaluation: 1) Upon application, the budget might be fixed and the QM is required to generalize out-of-the-box to this setting. 2) We are interested in the minimal budget at which the QM works since a too large budget implies inefficient labeling (equivalent to random queries) and a too small budget is likely to cause AL failure (cold start problem). This search needs to be performed prior to an AL application due to the validation paradox. 


%
%
\textbf{P3: Lack of evaluated query sizes}
The number of samples queried for annotation per acquisition step is essential to a realistic evaluation of QMs. This is because, upon application, this parameter might be predefined by the compute-versus-label cost ratio of the respective task (a smaller query size amounts to more compute cost but might enable more informed queries and thus less labeling). Since query size cannot be validated on the task at hand due to the validation paradox, the generalizability of QMs to various settings of this parameter needs to be evaluated beforehand.


%
\textbf{P4: Neglection of the classifier configuration}
% if in Section is wished use: \Cref{ss:realistic-eval}
As stated in \cref{ss:realistic-eval}, when aiming to draw conclusions about the performance or usefulness of a QM, it is critical that this evaluation be based on well-configured classifiers. Otherwise, performance gains might be attributed to AL that could have been achieved by simple HP modifications. Separating a validation split from the training data is a crucial requirement for sound HP tuning.


%

%
%
\textbf{P5: Neglection of alternative training paradigms}
Analogously to arguments made in P4, meaningful evaluation of AL requires comparison against alternative approaches that address the same problem. Specifically, the training paradigms Self-SL \cite{chenSimpleFrameworkContrastive2020a, heMomentumContrastUnsupervised2020} and Semi-SL \cite{sohnFixMatchSimplifyingSemisupervised2020, leePseudolabelSimpleEfficient2013} have shown strong potential to make efficient use of an unlabeled data pool in a classification task thus alleviating the labeling burden. Additionally to benchmarking AL against Self-SL and Semi-SL, the question arises of whether AL can yield performance gains when combined with these paradigms.



\subsubsection{Contrasting Research with Practice}
When applying AL on a new, mostly unlabelled data set, one can not directly validate whether QM1 or QM2 performs better, as this would require labeling individual AL trajectories through the data set for each QM. This excessive labeling would directly contradict the goal of AL to reduce labeling (“validation paradox”). 
Notably, this is in contrast to standard ML, where a fixed labeled validation split suffices to optimize the model configuration. Thus, the validation paradox forces one instead to estimate how well certain QMs will perform on the given task based only on prior knowledge. 
The quality of this estimate directly depends on the prior knowledge available, i.e. on how extensively the respective QM has been validated in the first place and how trustworthy the results are (close to realism). 
The application at hand typically comes with a given data distribution which is not necessarily a balanced object recognition task (P1) and possible constraints on the size of the starting budget (P2) and the query size (P3) due to labeling or training cost. 
However, at the very least, the practitioner wants to know how to set them so that Active Learning will yield benefits.
Also, the practitioner will try to label as little as possible to solve the task and, therefore will rigorously tune the hyperparameters of his models from a set of training schemes (e.g. Standard Training, Self-Supervised Pretrained or Semi-supervised) to ensure the best performance of his model for a given amount of annotations, or at the very least a good cost to performance ratio.
To do this, he will also require a validation set based on which he determines the final setup of his model.

Whereas in research, most evaluations presenting AL methods focus on a very limited amount of datasets which are not representative of the wide amount of data distributions found in many real world tasks. Further, often the methods are also developed on these datasets which has a high potential of overfitting a QM to these datasets.
Mostly only a very specific range of starting budgets and query sizes is evaluated while also not tuning the hyperparameters of their models using a validation sets.
Further, evaluation of alternative training schemes is also not the standard.



% Version showing pitfalls but very strong doubling with the pitfalls.
% \subsubsection{Pitfalls in Practice}
% When applying AL on a new, mostly unlabelled data set, one can not directly validate whether QM1 or QM2 performs better, as this would require labeling individual AL trajectories through the data set for each QM. This excessive labeling would directly contradict the goal of AL to reduce labeling (“validation paradox”). 
% Notably, this is in contrast to standard ML, where a fixed labeled validation split suffices to optimize the model configuration. Thus, the validation paradox forces one instead to estimate how well certain QMs will perform on the given task based only on prior knowledge. The quality of this estimate directly depends on the prior knowledge available, i.e. on how extensively the respective QM has been validated in the first place. 
% The application at hand typically comes with a given data distribution (P1) and constraints on the size of the starting budget (P2) and the query size (P3) where changing either one of these two parameters can lead to different annotation trajectories. 
% To ensure that the prior knowledge about the performance of a QM covers such specific application constraints, the QM needs to be validated on a realistic range of all of these parameters. Not doing so causes P1-P3 and limits the reliability of the required performance estimates of a QM in practice. 
% Further, since AL adds costs over random annotation, assessing the practical value of a QM must include comparison against alternatives. For instance, if the gain of a QM over random sampling can also be achieved by simply tuning the learning rate of the classifier, the QM provides no practical value (P4), and similarly, if the gain can be achieved by a single SSL pretraining, the QM provides no practical value either (P5). 
% Finally, several hyperparameters have to be configured in AL application, like the classifier configuration (P4), but also possible hyperparameters of the QM itself. 

% Leave out
% Since it is not feasible to validate a QM for all settings in this high-dimensional parameter space, as required by the validation paradox, we instead propose to test the robustness of a few optimized settings on additional datasets (“roll-out datasets”) that were not part of the optimization process (“development datasets”). Taken together, statements about the practical value of a QM require addressing all five pitfalls P1-P5 and testing on “roll-out datasets”.

\subsubsection{Proposed evaluation Framework}
\textbf{P1}
Increase the number of datasets on which AL is evaluated by using real-world tasks and also incorporate class imbalances. 
Further, we propose to split the available datasets into "roll-out" and "developmental" datasets to allow testing the robustness of AL methods in novel settings (roll-out dataset) where the selection of hyperparameters of both QM and classifier has to follow clear rules without inferring knowledge from previous AL trajectories on these datasets. In contrast to the development datasets where these rules are inferred from.

% Old P1
% \textbf{Proposed solution:} We argue that the underrepresentation of class-imbalanced datasets in the field is one reason for current doubts regarding the general functionality of AL. Real-life settings will most likely not be class balanced providing a natural advantage of AL over random sampling. We propose to consider diverse datasets with real class imbalances as an essential part of AL evaluation and advocate for the inclusion of "roll-out" datasets, as a real-life test of selected and fixed AL settings.


\textbf{P2 \& P3} 
We evaluate all QMs for three different starting budgets and query sizes on all datasets with three respective \textit{label regimes} (low-, mid-, and high). Extending on the findings of \cite{bengarReducingLabelEffort2021a}, the starting budgets and query sizes are determined using heuristics based on the number of classes per task.
Of special interest is here the low- and mid-label regime which are more susceptible to fall prone to the cold-start. 
We deem both starting budget size and query size together as a fair tradeoff to make experiments feasible, as theory shows that adapted smaller query size for the low label regime can only positively affect the result compared to a larger query size \cite{kirschBatchBALDEfficientDiverse2019a} and we are not aware of any work claiming that large query size hurts performance. 
Therefore, we could interpret the performance of a small starting budget too positively due to a hidden effect of the smaller query size.
However, we also study the effect of query size in the low-label settings directly, where we perform an additional ablation with varying query sizes on a small fixed starting budget.




\textbf{P4}
To enable a meaningful performance assessment of AL methods, we define a validation dataset of a size deducted heuristically from the starting budget. Based on this data, a small selection of HPs (learning rate, weight decay and data augmentations \cite{cubukRandaugmentPracticalAutomated2020}) is tuned only once per AL experiment while training on the starting budget. The limited search space and discarding of multiple tuning iterations result in a lightweight and practically feasible protocol for classifier configuration.

% Old P4
% \textbf{Proposed solution:} To overcome this pitfall and enable meaningful performance assessment of AL methods, we define a validation dataset of a size deducted heuristically from the starting budget. Based on this data, a small selection of HPs (learning rate, weight decay and data augmentations \cite{cubukRandaugmentPracticalAutomated2020}) is tuned only once per AL experiment while training on the starting budget. The limited search space and discarding of multiple tuning iterations result in a lightweight and practically feasible protocol for classifier configuration.

\textbf{P5}
To resolve current inconsistencies, we benchmark all QMs against  both Self-SL and Semi-SL, and evaluate the combination of AL with these paradigms. Crucially, we are the first to study these relations in a trustworthy setting, i.e. while avoiding all other key pitfalls of realistic AL evaluation (P1-P4).

% \textbf{Proposed solution:} To overcome this pitfall and resolve current inconsistencies, we benchmark all QMs against  both Self-SL and Semi-SL, and evaluate the combination of AL with these paradigms. Crucially, we are the first to study these relations in a trustworthy setting, i.e. while avoiding all other key pitfalls of realistic AL evaluation (P1-P4).

==> tex/99_depr_tex/03_methods.tex <==
In supervised learning, we are given a labeled dataset of observation-target pairs $(x,y) \in \mathcal{L}$ sampled from an unknown joint distribution $p(x,y)$. 
Our goal is to produce a prediction function $f_\theta(x)$, parameterized by $\theta$, which outputs a target value for previously unseen samples from $p(x)$. 
Choosing $\theta$ might amount, for example, to optimizing a loss function which reflects the extent to which $f_\theta(x)=y$ for $(x,y) \in \mathcal{L}$. 
However, in pool-based AL we are additionally given a collection of unlabeled observations $\mathcal{U}$, sampled from $p(x)$. 
By using a query method, we hope to leverage this data efficiently through querying and successively labeling the most informative observations $(x_1, ... x_B)$ from the pool, leading to a prediction function which is more accurate on the newly created labeled set than if random observations were queried.
\\
From a more abstract perspective, the goal of AL is to use the information of the labeled dataset $\mathcal{L}$ and the prediction function $f_\theta(x)$, to find the observations giving the most information where $p(y|x)$ deviates from $f_\theta(x)$. 
This is also being reflected by the way performance in AL is measured -- which is the relative performance gain of the prediction function with queries from a query method compare to random queries.
Making the prediction function implicitly the gauge for measuring the "success" of an AL strategy.
\\
A comprehensive overview over AL and its methods is out of the scope of this paper, we refer interested readers to \cite{}. 
Instead, we focus on the class of query methods which solely use the prediction function as a basis for their queries, and otherwise leave the training-strategy and model unchanged.
In addition, methods belonging to this category currently hold the state-of-the-art in AL on classification tasks, while also being operational less complex to implement. 
Further, they require no additional HPs to be set for the query function which is hard to evaluate in practice due to the validation paradoxon.\\

Overall, the methods we consider fall into two classes: explorative strategies, which enforce queried observations to explore the distribution of $p(x)$; and uncertainty based strategies, which make direct use of the prediction function $f_\theta(x)$.
\footnote{This is conceptually similar to the exploration and exploitation paradigm seen in Reinforcement Learning and there actually exist strong parallels between Reinforcement Learning and Active Learning -- so much so that Reinforcement Learning has been proposed to use in AL and AL based strategies have been proposed to be used in Reinforcement Learning.}
The principled combination of both strategies, especially to allow higher query sizes for uncertainty based query methods, is an open research question.\\

In this section, we describe the applied methods in more general terms and refer to \cref{app_s:qm} for a detailed review.
\paragraph{Random:} The simplest query method possible includes drawing observations randomly from $\mathcal{U}$ and therefore following $p(x)$, deeming it as an explorative strategy.
\paragraph{Core-Set:} This method is based on the finding that the decision boundaries of convolutional neural networks are based on a small set of samples. To find these observations, the Core-Set approach queries observations which minimize the maximal shortest path from unlabeled to labeled sample in the representation space of the classifier \cite{senerActiveLearningConvolutional2018b}. This is also known as the K-Center problem, for which we use the K-Center greedy approximation. It draws queries especially from tails of the data distribution, to cover the whole dataset as well as possible. Therefore we classify it as an explorative strategy.
\paragraph{Entropy:} Makes use of the uncertainty of a prediction for a sample given by the prediction function.
% Captures the uncertainty of the prediction of the classifier by using the entropy of the classifier output.
\paragraph{BALD:} Aims to query observations with the highest mutual information between the class label variable $Y$ and the weights $\theta$ \cite{houlsbyBayesianActiveLearning2011}, which was introduced with dropout for deep bayesian active learning by \cite{galDeepBayesianActive2017a}.
\paragraph{BatchBALD:} Is an extension of BALD and aims to query a batch $(x_1, ..., x_B)$ with the highest joint mutual information between the batch of class labels $Y_1, ..., Y_B$ and the weights $\theta$ \cite{kirschBatchBALDEfficientDiverse2019a}.

\subsection{Self-Supervised (Learning) Pre-Training}\label{sec:03-selfsl}
The high-level concept of Self-SL pre-training is to obtain a model by training it with a proxy task which is not dependent on annotations leading to representations that generalize well to a specific task.
This allows to induce information from unlabeled data into the model in form of an initialization which can be interpreted as a form of bias.
Usually these representations are supposed to be clustered based on some form of similarity which is often induced directly by the proxy task and also the reason why different proxy tasks are useful for different downstream tasks.
Several different Self-SL pre-training strategies were developed based on different tasks s.a. generative models or clustering \cite{}, with contrastive training being currently the de facto standard in image classification.
Based on this, we use the popular contrastive SimCLR \cite{chenSimpleFrameworkContrastive2020a} training strategy as a basis for our Self-SL pre-training.
% For Self-Supervised Pre-Training we choose SimCLR \cite{chenSimpleFrameworkContrastive2020a}, since it is a simple, commonly known and widely used self-supervised pre-training strategy. It works by... Contrastive Cluster Building
\subsection{Semi-Supervised Learning}\label{sec:03-semisl}
In Semi-SL the core idea is to regularize $f_\theta(x)$ by inducing information about the structure of $p(x)$ of the unlabeled pool in combination with the labeled dataset.
Usually this leads to the representations of unlabeled observations being more clustered according to the prediction structure of the supervised task.
Several different Semi-SL methods were developed based on regularizations on unlabeled observations which often fall into the category of enforcing consistency of predictions against perturbations and/or reducing the uncertainty of predictions \cite{}. 
\footnote{It is also a fair argument that Self-SL pre-trained models is also a form of Semi-SL if finetuned on a small labeled subset.}
In our experiments we use FixMatch \cite{sohnFixMatchSimplifyingSemisupervised2020} as Semi-SL method which combines both aforementioned principles of consistency and uncertainty reduction in a simple manner.
% For Semi-Supervised Learning we chose FixMatch \cite{sohnFixMatchSimplifyingSemisupervised2020} due to its simplicity and state-of-the-art results on CIFAR-10 and CIFAR-100. It works by.... Cluster Hypothesis \& Instability?

==> tex/99_depr_tex/05_depr_results.tex <==
Here we will discuss the results for each of the individual datasets, so as to let the reader draw their own conclusions and/or agree disagree with our interpretation which we will then again present structured for our different improvements.
\subsection{Main Experiments}
These experiments represent the main evaluation for Active Learning strategies based on the improvements discussed in section 2 and the exact setup described in section 3.
They should give an answer to the question "In which settings AL is beneficial for Deep Classification?" by using multiple different settings to evaluate the generalizability and find patterns for performance.\\
The results are ordered by the datasets and describe how AL performs with each of the three training strategies on each of the three different label regimes.
% should compare the effect of Active Learning in combination with a wide array of different settings, to verify their generalizability or find underlying patterns for their performance.
\paragraph{General Observations}
The overall performance level of models for a setting was determined by: 1. The training strategy and 2. the hyperparameter selection.
The benefits of using AL we observed, were generally smaller compared to proper selection of 1 and 2.
\paragraph{CIFAR-10} 
Training Strategy defines the overall performance and AL does finetuning across the three different regimes.\\
Best Sem-SL, Self-SL and then Supervised. All results can be seen in \autoref{fig:acc-cifar10-full}.\\
% This line might need to be rewritten!
For Sem-SL training (\autoref{fig:app-cifar10-full-SemSL}) there is no clear trend whether AL benefits the model. 
For Self-SL pre-trained models gain on all stages from some AL significantly. The explorative Core-Set approach brings benefits in the low-label regime and medium-label regime.
However, for the high-label regime the uncertainty based strategies Entropy and BALD perform best (\autoref{fig:app-cifar10-full-SelfSL})\\
BALD and Entropy seem to suffer from the cold-start problem for the low-label regime (this is interesting due to the model performing well and acq. size being small (rel. to applied literature)!)\\
For our supervised models, AL only brings benefits for the high label regime with Entropy performing significantely worse in the low and medium label regimes.
Core-Set and BALD perform as good as random on medium and low label regime, and while the final performance is very similar for Core-Set and BALD, Core-Set is over the whole AL setting more robustly performing significantely better than random (\autoref{fig:app-cifar100-full-basic}).\\
% Add part about performance of our supervised model when compared to AL literature?
\paragraph{CIFAR-100}
Overall plot can be seen in \autoref{fig:acc-cifar100-full}.
Training Strategy also defines overall performance and AL does finetuning. 
Sem-SL with ResNet18 does not perform so much better than Self-SL.
For Sem-SL no AL strategy seems to bring benefit (\autoref{fig:app-cifar100-full-SemSL}). \\
For Self-SL models on low and medium label regime there are no benefits, Core-Set close to random and Entropy and BALD perform worse.
In the high label regime, AL starts to bring benefits, Core-Set and BALD perform similar and Entropu performs best (\autoref{fig:app-cifar100-full-SelfSL}). \\
For Basic in the low and medium label regime, BALD and Core-Set perform on a level with random, while Entropy performs signifantely worse.
In the high label regime for the final value uncertainty based BALD and Entropy perform best while over the whole plot BALD performs best, followed by Core-Set.(\autoref{fig:app-cifar100-full-basic}) \\ 
% Add part about performance of our supervised model when compared to AL literature?
\paragraph{CIFAR-10 LT}
Full Plot (\autoref{fig:acc-cifar10-LT-full})
Training Strategy also defines overall performance and AL does finetuning. 
Sem-SL with ResNet18 starts performing better for more labels.
AL can bridge gap between Self-SL pretrained models and Basic models on medium label regime and can make it outperform for high label regime.\\
% Possilby Sem-SL has to be rewritten.
For Sem-SL in low label regime, AL performs similar to random. For the medium label regime Core-Set outperforms random possibly due to drawing samples making the model more stable. (\autoref{fig:app-cifar10LT-full-SemSL}) \\
For Self-SL models BALD brings benefits for all three regimes. Entropy brings benefits similarly and Core-Set starts to bring benefits from the medium label regime onward.  (\autoref{fig:app-cifar10LT-full-SelfSL}) \\
For Basic models Core-Set brings advantages over all label regimes, BALD for low and medium label while Entropy performs similar or a little worse to random. 
BALD does not recover in the high label regime.(\autoref{fig:app-cifar10LT-full-basic}) 
\paragraph{MIO-TCD}
Full Plot (\autoref{fig:bAcc-miotcd-full}) in the high label regime AL (Core-Set) leads to basic models performing on par/outperforming Self-SL.
Sem-SL ... (models performed absolutely terrible and are therefore omitted -- info in table XYZ).\\
For Self-SL models no AL strategy significantely outperforms random. BALD performs much worse than all other strategies. (\autoref{fig:app-miotcd-full-SelfSL}) \\
For Basic models Core-Set outperforms random sampling for all regimes, Entropy performs worse than random for all regimes and BALD performs better for medium (and high), while performing worse for low label regime. (\autoref{fig:app-miotcd-full-basic})
\paragraph{ISIC-2019}
Full Plot (\autoref{fig:bAcc-isic2019-full}) in the med label regime AL (Core-Set) leads to basic models getting very close to Self-SL models.
Sem-SL ... (models performed absolutely terrible and are therefore omitted -- info in table XYZ).\\
For Self-SL models BALD performs best for the low and medium label regime. In the high label regime it starts to perfom worse at a 2.2k samples.
In the low-label regime neither entropy or Core-Set outperform random. In the medium and high label regime Entopy outperforms random and Core-Set performs as good as random. (\autoref{fig:app-isci2019-full-SelfSL})\\
In the low label regime there is only noise for Basic models with a tendency for Core-Set to outperform random. In the medium and high label regime Core-Set significantely outperforms random, while Entropy performs on the same level while BALD has a tendency to perform worse. (\autoref{fig:app-isci2019-full-basic}).

\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        % \includegraphics[width=\linewidth]{"PaperDraftv2/CIFAR-10/acc-full.png"}
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-full_train-all.pdf}
        \caption{CIFAR-10 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
        \label{fig:acc-cifar10-full}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-full_train-all.pdf}
        \caption{CIFAR-100 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
        \label{fig:acc-cifar100-full}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-full_train-all.pdf}
        \caption{CIFAR-10 LT Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
        \label{fig:acc-cifar10-LT-full}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        % \includegraphics[width=\linewidth]{"PaperDraftv2/Mio-TCD/mRe-full.png"}
        \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-full_train-all.pdf}
        \caption{MIO-TCD Mean Recall. }
        \label{fig:bAcc-miotcd-full}
    \end{subfigure}
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-full_train-all.pdf}
        \caption{ISIC-2019 Mean Recall Dip in Performance is ablated in the Appendix....}
        \label{fig:bAcc-isic2019-full}
    \end{subfigure}
\end{figure*}
% \begin{figure}
%     \centering
%     % \includegraphics[width=\linewidth]{"PaperDraftv2/CIFAR-10/acc-full.png"}
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-full_train-all.pdf}
%     \caption{CIFAR-10 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%     \label{fig:acc-cifar10-full}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-full_train-all.pdf}
%     \caption{CIFAR-100 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%     \label{fig:acc-cifar100-full}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-full_train-all.pdf}
%     \caption{CIFAR-10 LT Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%     \label{fig:acc-cifar10-LT-full}
% \end{figure}
% \begin{figure}
%     \centering
%     % \includegraphics[width=\linewidth]{"PaperDraftv2/Mio-TCD/mRe-full.png"}
%     \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-full_train-all.pdf}
%     \caption{MIO-TCD Mean Recall. }
%     \label{fig:bAcc-miotcd-full}
% \end{figure}
% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-full_train-all.pdf}
%     \caption{ISIC-2019 Mean Recall Dip in Performance is ablated in the Appendix....}
%     \label{fig:bAcc-isic2019-full}
% \end{figure}

\subsection{Cold-Start Low-Label Ablation}
These experiments were conducted in the low-label regime to assess the importance of acquisition size for Self-SL pre-trained models and gain insights on the Cold-Start problem.
Since the performance of Self-SL models with Active Learning is not as steady as we would have expected, especially for BALD.
Therefore we additionally compare BatchBALD since it should behave more like a model where single data points are drawn per AL iteration and with the good initial model performance this should circumvent the Cold-Start problem.
\paragraph{CIFAR-10} BatchBALD is best performing strategy, significantely better than random and BALD, it performs as good as Core-Set.
\paragraph{CIFAR-10-LT} BatchBALD performs as good as BALD and is best performing strategy.
\paragraph{CIFAR-100} due to the smaller acquisition size all AL strategies perform better. Core-Set and BALD are best strategies. BALD performs a little better than random and Entropy a little worse.
\paragraph{MIO-TCD} the random pre-sampling of the pool leads to BALD performing significantely better. BatchBALD outperforms both Core-Set and random on all stages.
Core-Set seems to suffer from the pre-selection same as entropy, later of which does so significantely.
\paragraph{ISIC-2019} BatchBALD performs as good or a little bit better than BALD, and therefore is the best performing strategy.


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-10}
        \label{fig:cifar10-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-10 LT}
        \label{fig:cifar10-LT-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-low-bb_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-100 (small acq. size)}
        \label{fig:cifar100-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-low-bb-fulll_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{MIO-TCD (small Pool)}
        \label{fig:mio-tcd-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{ISIC-2019 }
        \label{fig:isic2019-bb}
    \end{subfigure}
    \caption{Low Label Ablations to verify the influence of acquisition size with BatchBALD.}
\end{figure*}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
%     \caption{CIFAR-10 Low Label Ablation with BatchBALD}
%     \label{fig:cifar10-bb}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
%     \caption{CIFAR-10 LT Low Label Ablation with BatchBALD}
%     \label{fig:cifar10-LT-bb}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-low-bb_train-Self-SL_yshared-False_bound-False.pdf}
%     \caption{CIFAR-100 Low Label with smaller acquisition size: Ablation with BatchBALD}
%     \label{fig:cifar100-bb}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-low-bb-fulll_train-Self-SL_yshared-False_bound-False.pdf}
%     \caption{MIO-TCD Low Label Ablation with BatchBALD}
%     \label{fig:mio-tcd-bb}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
%     \caption{ISIC-2019 Low Label Ablation with BatchBALD}
%     \label{fig:isic2019-bb}
% \end{figure}



==> tex/99_depr_tex/05_results.tex <==
Here we will discuss the results for each of the individual datasets, so as to let the reader draw their own conclusions and/or agree disagree with our interpretation which we will then again present structured for our different improvements. 

\subsection{Main Experiments}
These experiments represent the main evaluation for Active Learning strategies based on the key parameters discussed in \cref{sec:relworks} query methods and Self-SL and Semi-SL training strategies from \cref{sec:methods} and the exact setup described in \cref{sec:experiments}.
They answer the question "In which settings AL is beneficial for Deep Classification?" by using multiple different settings to evaluate the generalizability and find patterns with regard to the  performance of query methods compared to random.
The results for all main experiments are shown in \cref{fig:main-exp} with detailed plots for each training strategy and label regime in the appendix X.
% The results are ordered by the datasets and describe how AL performs with each of the three training strategies on each of the three different label regimes.
% should compare the effect of Active Learning in combination with a wide array of different settings, to verify their generalizability or find underlying patterns for their performance.
\\
\textbf{General Observations:}
% \paragraph{General Observations}
For all datasets the overall performance of models was primarily determined by the training strategy and the hyperparameter selection, with the benefits of AL being generally smaller compared to proper selection of both.
For the three toy datasets Semi-SL generally performed best, followed by Self-SL and ST last, whereas for the two real-world datasets Semi-SL showed no significant improvement over ST in the first training stage and therefore further runs were omitted.
Also the performance gains for Self-SL models with AL are generally smaller compared to ST models. 
For Semi-SL there were generally only very small performance gains or significantly worse performance with AL observed.
With regard to the effect of AL, the high-label regime proved to work for ST models on all datasets and for Self-SL models.
On the two real-world datasets MIO-TCD and ISIC-2019 a dip in performance at ~7k samples for all ST models could be observed. 
This is ablated in the appendix and can be traced back to our choice of HPs.
\\
\textbf{CIFAR-10:}
Semi-SL showed the biggest benefits being already close the performance of our ST classifier on the whole dataset for 50 labeled observations.
Self-SL pre-trained models gain on all stages from AL significantely with explorative Core-Set bringing benefits in the low- and medium-label regime, whereas for the high-label regime the uncertainty based query methods BALD and Entropy perfoorm best.
For ST models AL only brings benefits in the high label regime where Core-Set performs best, followed by BALD and Entorpy being the overall worst query method even having areas with significantly worse performance than random queries.
\\
\textbf{CIFAR-100:}
Semi-SL performs very similar to Self-SL on low-label regime and only outperforms it in the medium-label regime. Also for Semi-SL models random queries perform significantly better than all AL strategies.
For Self-SL models all query methods except for Core-Set perform significantly worse than random queries for the low- and medium-label regimes, whereas in the high label regime all AL methods significantly increase performance with Entropy being the best followed by Core-Set and BALD with almost equal performance.
A similar trend can be observed for ST models with the difference that the Entropy query method is the only one leading to a significant drop in the low- and medium-label regime and BALD performing best for the high-label regime. Core-Set has a better performance in the beginning but being overtaken by Entropy leading to similar performance than uncertainty based BALD. 
\\
\textbf{CIFAR-10 LT:}
Performance of Semi-SL is spread widely in the low label regime and Core-Set seems to bring benefits especially in the medium-label regime where models become worse, this performance difference could be reduced by selecting the model checkpoint with the highest validation accuracy.
For Self-SL models entropy brings benefits for three label regimes being the overall best query method, followed by Entropy and Core-Set which performs (non-significantely) worse than random.
ST models signficantely benefit from AL on all three label regimes with Core-Set bringing benefits for all and BALD bringing benefits for the low- and medium- label regime, whereas Entropy generally performs worse than random.
\\
\textbf{MIO-TCD:}
For Self-SL models no query method signficantely outperforms random with BALD performing much worse than everything else.
For ST models Core-Set outperforms random on all three label regimes, Bald leads to benefits in the medium-label regime and is inconsistent in the high label regime while Entropy performs worse than random on all three label regimes.
Core-Set ST performs as well as Self-SL models in final stage of the high-label regime.
\\
\textbf{ISIC-2019}
For Self-SL models BALD leads to performance gains in the low- and medium-label regime while dropping off later in the high-label regime and Entropy brings benefits in the medium- and high-label regime. Core-Set performs inconsistently as well or worse than random queries.
For ST models Core-Set leads to performance gains on all three label-regimes with Entropy and BALD generally performing worse than random queries.
Core-Set closes the performance difference between Self-SL and ST in the medium (\& potentially high) label-regime.

% \begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.495\textwidth}
%         \centering
%         % \includegraphics[width=\linewidth]{"PaperDraftv2/CIFAR-10/acc-full.png"}
%         \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-full_train-all.pdf}
%         \caption{CIFAR-10 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%         \label{fig:acc-cifar10-full}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.495\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-full_train-all.pdf}
%         \caption{CIFAR-100 Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%         \label{fig:acc-cifar100-full}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.495\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-full_train-all.pdf}
%         \caption{CIFAR-10 LT Test Accuracy. Training+Pool Dataset consists of 45.000 samples and Validation Dataset of maximal 5.000 datapoints.}
%         \label{fig:acc-cifar10-LT-full}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.495\textwidth}
%         \centering
%         % \includegraphics[width=\linewidth]{"PaperDraftv2/Mio-TCD/mRe-full.png"}
%         \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-full_train-all.pdf}
%         \caption{MIO-TCD Mean Recall. }
%         \label{fig:bAcc-miotcd-full}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.495\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-full_train-all.pdf}
%         \caption{ISIC-2019 Mean Recall Dip in Performance is ablated in the Appendix....}
%         \label{fig:bAcc-isic2019-full}
%     \end{subfigure}
%     \caption{Main Experiments}
%     \label{fig:main-exp}
% \end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{deep-active-plots/main/Deep-Results.pdf}
    \caption{Main Experiments}
    \label{fig:main-exp}
\end{figure*}

\subsection{Cold-Start Low-Label Ablation}
In this ablation the importance of the query size was ablated with regard to Self-SL models.
This was insprired by our observations of models with good performance and (in comparison to practical literature) small query sizes not benefitting from AL strategies which is commonly attributed to the cold-start problem.
Our evaluation uses BatchBALD since it simulates smaller acquisisiton sizes for BALD. Based on this for CIFAR-100 query size was lowered to 50 while for MIO-TCD the size of the pool was artificially reduced to 50k at each query step -- both to lower the computational cost of BatchBALD.
\\
The results are shown in \cref{fig:bb-exp} where it clearly shows that first BatchBALD always performs better or as good as BALD. Where the simulated smaller query size of BatchBALD making the difference between performing better or worse than random on all datasets except for ISIC-2019, where BALD already is the best performing query method.\\
Further on CIFAR-100 the reduced query size benefits all query methods and for MIO-TCD the smaller pool signficantely improves the performance of BALD (comparison in appendix ).


\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-10}
        \label{fig:cifar10-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-10-LT/Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-10 LT}
        \label{fig:cifar10-LT-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/CIFAR-100/Accuracy/plot-low-bb_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{CIFAR-100 (small acq. size)}
        \label{fig:cifar100-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/MIO-TCD/Balanced-Accuracy/plot-low-bb-fulll_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{MIO-TCD (small Pool)}
        \label{fig:mio-tcd-bb}
    \end{subfigure}
    \begin{subfigure}[b]{0.195\textwidth}
        \centering
        \includegraphics[width=\linewidth]{deep-active-plots/ISIC-2019/Balanced-Accuracy/plot-bblow_train-Self-SL_yshared-False_bound-False.pdf}
        \caption{ISIC-2019 }
        \label{fig:isic2019-bb}
    \end{subfigure}
    \caption{Low Label Ablations to verify the influence of query size with BatchBALD.}
    \label{fig:bb-exp}
\end{figure*}
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{deep-active-plots/main/BatchBALD.pdf}
    \caption{Low Label Ablations to verify the influence of query size with BatchBALD.}
    \label{fig:bb-exp}
\end{figure*}




==> tex/99_depr_tex/06_depr2_discussion.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{deep-active-plots/main/Deep-Results.pdf}
    \caption{Main Experiments}
    \label{fig:main-exp}
\end{figure*}

In this section, we will start by a discussion of our key parameters (K1-K5) and the advantages gained through our improved AL evaluation protocol, followed by general insights we were able to extract from our experiments and setting them into relation with related works. \\
Finally we end with the limitations of our work.\\
% Start discussing experiments
Our experiments were conducted as follows: First, we started by running experiments with the proposed label regimes and all settings described in \cref{sec:experiments}, results are shown in \cref{fig:main-exp}. 
% Start BatchBALD Discussion
However, we were so confused about the results of Self-SL models in the low-label regime that we ran an ablation study with regard to the query size on all datasets additionally using BatchBALD as query method, results are shown in \cref{fig:bb-exp}. 
Further, in this ablation changes were made for CIFAR-100 (query size was changed form 500 to 50) and for MIO-TCD (pool was downsampled by random sampling 50000 observations) to have reasonable runtimes with BatchBALD.
\subsection{Discussion of Key-Parameters with our Evaluation Protocol}
Here, we will set all results of our experiments into context of the five key-parameters and discuss it with regard to our main insights (F1-F...) generated of our evaluation protocol.
% in a fashion structured by our proposed improvements to the evaluation of AL methods for our key parameters.


\paragraph{K1 Data Distribution}
The different label distributions in our experiments proved to be one of the most important parameters w.r.t. the performance of AL. Indeed could this result been anticipated, as the dataset is also the most important parameter for setting up a well performing model in general. For the class imbalanced datasets, AL seems to bring the highest benefit compared to random queries. 
% This might also hint towards the use-case of simple baselines and new query methods enforcing label uniformity by their design as among others proposed by \cite{krishnanImprovingRobustnessEfficiency2021}.

\paragraph{K2 Starting Budget}
The effect of differing starting budgets mostly leads to changes in the initial performance of the model but for our two real-world datasets the corresponding validation dataset sizes lead to different hyperparameter settings being selected.
The effect of different starting budgets on AL however can only be evaluated if combined with the query size (discussed in the next paragraph).
% and the validation set sizes are in case of the toy datasets mostly a performance difference but proved to be an important parameter, especially when combined with the query size (discussed in the next paragraph).\\
Our results indicate, that AL brings benefit with much smaller starting budgets than previously reported \cite{bengarReducingLabelEffort2021a, gaoConsistencyBasedSemisupervisedActive2020, mittalPartingIllusionsDeep2019a}, if set up correctly. 
These findings are especially true if combined with Self-SL, similar to the approach shown in \cite{tranPlexReliabilityUsing2022}. 
% This opens up the direction of experiments similar to the ones performed on toy experiments
\paragraph{K3 Query Size}
The effect of the query size appears to be different at different stages of the training and labeled set. 
In the high-label regime, there are (almost) always clear benefits of AL strategies whereas for the low- and medium-label regime this is not the case. Even for the Self-SL and Semi-SL models this can be observed, where the model performance should not lead to the Cold-Start problem. 
This observation is consistent with the literature \cite{bengarReducingLabelEffort2021a, gaoConsistencyBasedSemisupervisedActive2020, mittalPartingIllusionsDeep2019a}, but they do not take the query size as a key parameter with regard to this behavior (Cold-Start) into account.
Further, it is of special interest why AL only brings consistent benefits on all datasets in the high label regime in our experiments and the literature with query size being a non-crucial parameter \cite{munjalRobustReproducibleActive2022a}.
Based on our results and theoretically, the influence of each individual queried observation is the smallest in this case.
However, this might also explain this behavior since in label regimes where the model is subject to strong changes, random sampling might be better than structured sampling, where the model queries too many observations containing the same information. 
This might explain the strong performance of Core-Set in the low-label regime through enforcing exploration, but possibly also leading to bad performance on imbalanced datsets due to a high amount of samples being queried from the tails of the distribution.\\
The ablation experiments based on Self-SL models with BatchBALD, which effectively simulates a smaller query size with BALD, show that this always outperformed random queries for the low-label regime and improved over the performance of BALD.
% (even though the query size was even smaller for CIFAR-100 and for MIO-TCD the pool was shrinked by random sampling both of which steps improved however the performance of BALD for their respective datasets).
This supports the hypothesis, that BatchBALD efficiently alleviates the problems of first, oversampling specific regions in the observation space corresponding to a class (based on CIFAR-100), and second, sampling too similar observations (based on MIO-TCD) \cite{kirschBatchBALDEfficientDiverse2019a} making it in our opinion the most versatile query method if it were not computationally so expensive.
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{deep-active-plots/main/BatchBALD.pdf}
    \caption{Low Label Ablations to verify the influence of query size with BatchBALD.}
    \label{fig:bb-exp}
\end{figure*}

\paragraph{K4 Method Configuration}
Optimizing the hyperparameters of models with a validation set is to a large extend the most crucial step to obtain good performing models, even more than the inclusion of AL. For SL models difference in performance can be as high as a factor of five for the labeled training set, and similar observations hold true for Self-SL and Semi-SL models. 
When applying the commonly benchmarked settings, our supervised models outperformed on both CIFAR-10 and CIFAR-100 all random SL baselines, with the exception of \cite{munjalRobustReproducibleActive2022a} on CIFAR-100, where our performance is very similar but achieved with a much smaller budget for hyperparameter optimization.


\paragraph{K5 Methodological Context}
\textbf{Self-SL} brings advantages for all label regimes and datasets that were investigated, confirming the results of \cite{bengarReducingLabelEffort2021a}. 
In some cases the supervised baseline with AL even comes very close or outperforms Self-SL models (see CIFAR-10 LT and MIO-TCD in the high label regime). 
This might be due to a sub-optimal optimization routine for our Self-SL models on bigger dataset sizes and less influence of the pre-trained initialization.
In our hyperparameter sweeps Self-SL pre-trained models were remarkably stable with regard to optimal hyperparameter choices.
\\ 
\textbf{Semi-SL} brings the biggest advantages on less complex datasets s.a. CIFAR-10 and CIFAR-10 LT. On CIFAR-100 it performed marginally better than Self-SL but much worse than the performance given by \cite{sohnFixMatchSimplifyingSemisupervised2020}.
We mostly attribute this to the change of the architecture from WRN 28-10 to ResNet-18 with a reduction of parameters by a factor of XX and the shortened training time by a factor of 5.
For the more complex datasets ISIC-2019 and MIO-TCD, the performance can be considered unsatisfactory, especially with regard to the training time which is XX time of SL. 
% --> Limitations
% A bad choice of hyperparameters could be one explanation, but we argue that in practice it would be very hard to set these hyperparameters since we already swept the parameters noted as the most important ones (WD and LR) in addition to the general setting which was already very beneficial with a large validation set following\cite{oliverRealisticEvaluationDeep2019}. 
% Further it is a well known problem that Semi-SL models have problems generalizing to imbalanced and possibly noisy datasets containing outliers \cite{oliverRealisticEvaluationDeep2019, boushehriSystematicComparisonIncompletesupervision2020, zenkRealisticEvaluationFixMatch2022}.
Therefore we believe that the conclusions drawn by \cite{gaoConsistencyBasedSemisupervisedActive2020, mittalPartingIllusionsDeep2019a} that Semi-SL makes AL almost `pointless' is only true if Semi-SL performs as well as on the datasets on which it was developed.
However, to draw final conclusions about Semi-SL one would need to make a large study comparing multiple different Semi-SL algorithms on a big benchmark, which we believe would be an interesting case-study and would allow to assess the use of Semi-SL algorithms much more realistically than the current evaluation protocol. 
\\
The relative gain through AL is smaller for training strategies s.a. Self-SL and Semi-SL than for SL models. This is expected since more information about the distribution of the pool is already inside of the model when comparing to SL models with random initialization. The results for Core-Set are irritating, since we assumed that the good representations obtained should generally allow for large performance gains (data is clustered better).
% This also points to the interesting research direction w.r.t. query methods making use of this information about the pool. 


\subsection{General Insights about AL}
\paragraph{K1 Data Distribution} This could be due to the fact, that AL strategies have a tendency to query batches with a more uniform label distribution and might also explain why random sampling is such a strong baseline on balanced datasets with little noise s.a. CIFAR-10 and CIFAR-100. This finding is consistent with the literature \cite{krishnanImprovingRobustnessEfficiency2021, munjalRobustReproducibleActive2022a, galDeepBayesianActive2017a}.
Further, could this result explain why AL has been shown on tasks s.a. segmentation and object detection to greatly reduce labeling effort \cite{}. Datasets for these tasks are notoriously imbalanced and the goal of balanced models is reflected in the evaluation metrics (often mean DICE and MAP).

\paragraph{K2 Starting Budget} 
These findings are especially true if combined with Self-SL, similar to the approach shown in \cite{tranPlexReliabilityUsing2022}. 

\paragraph{K3 Query Size}
The ablation experiments based on Self-SL models with BatchBALD, which effectively simulates a smaller query size with BALD, show that this always outperformed random queries for the low-label regime and improved over the performance of BALD.
% (even though the query size was even smaller for CIFAR-100 and for MIO-TCD the pool was shrinked by random sampling both of which steps improved however the performance of BALD for their respective datasets).
This supports the hypothesis, that BatchBALD efficiently alleviates the problems of first, oversampling specific regions in the observation space corresponding to a class (based on CIFAR-100), and second, sampling too similar observations (based on MIO-TCD) \cite{kirschBatchBALDEfficientDiverse2019a} making it in our opinion the most versatile query method if it were not computationally so expensive.

\paragraph{K4 Method Configuration}

\paragraph{K5 Methodological Context}
\subsection{Limitations}
The first and foremost limitation is the limitation to our evaluated settings (dataset, label regimes, hyperparameter optimization, training strategies). 
We cannot guarantee that our selected settings were optimal with regard to all compared training strategies, but comprises had to be made to compare everything, therefore our results (especially with regard to Self-SL and Semi-SL as end-users) have to be seen in the context of our limited setting.\\ 

% Method Configuration:
We acknowledge, that the size of our validation set might seem excessively large with a size of 5 times the starting budget, but we deemed proper validation of models to be essential for trusting a model to select queries for labeling. 
The experiments by \cite{munjalRobustReproducibleActive2022a} also show that a smaller validation set did only marginally change the performance of their models, thereby our results may also hold true for smaller validation set sizes.
Against our proposed hyperparameter selection scheme stands the dip in performance for all of our SL models on MIO-TCD and ISIC-2019 with ~7000 labeled observations. This is purely due to the choice of hyperparameter which we ablate in the appendix with random baselines. 
However we believe that this is mostly attributed to instabilities in the optimization due to the weighted loss since a small dip can also be observed for CIFAR-10 LT. In an ablation with SL models without weighted loss (see appendix) the performance was actually better and no such dip occurred.
Thus, for imbalanced datasets more optimal training strategies and methods to handle imbalanced label distributions should be evaluated (s.a. SMOTE) since efficient handling imbalanced datasets is crucial for the adaptation of AL as it represents a major use-case.
%  A more thorough and realistic approach in the training step would be to use K-Fold CV for hyperparameter tuning and also on each training step (this would also immediately give access to ensembles shown to be superior for uncertainties and also queries). However, due to the immense training cost of Semi-SL models, we did not implement this in this comparison.

% Semi-SL
A bad choice of hyperparameters could explain our unsatisfactory results with Semi-SL for the two real-world roll out dataset, but we argue that in practice it would be very hard to set these hyperparameters since we already swept the parameters noted as the most important ones (WD and LR) in addition to the general setting which was already very beneficial with a large validation set following\cite{oliverRealisticEvaluationDeep2019}. 
Further it is a well known problem that Semi-SL models have problems generalizing to imbalanced and possibly noisy datasets containing outliers \cite{oliverRealisticEvaluationDeep2019, boushehriSystematicComparisonIncompletesupervision2020, zenkRealisticEvaluationFixMatch2022}.

==> tex/99_depr_tex/06_depr_discussion_n_conclusion.tex <==
% \paragraph{FixMatch Problems} Semi-Supervised Learning is known to be problematic for imbalanced datasets... \cite{schmarjeSurveySemiSelf2021}. The cost of training just one Semi-Supervised model is generally X times higher than training one supervised model. With consistent retrainings it is X times higher than that of Self-SL PT models.
% \paragraph{Pre-Trained Models} We believe that finetuning based on either powerful pretrained models s.a. PLEX and/or Self-Supervised Learning are currently the most promising avenues for future Active Learning research.\\
% Based on: 1. Fast Training 2. Good performance with little data 3. Similarity of direction to BERT etc.

\subsection{Discussion}
\paragraph{Realistic Methodoligical Context}
\begin{itemize}
    \item Self-SL brought advantages for all label regimes and datasets we investigated in. \\
    Therefore we highly recommend the use of Self-SL on basically all datasets, especially due to its robustness of hyperparameters and models.\\
    In some cases models trained in a basic fashion performed as well as/outperformed Self-SL pretrained models. We believe that with proper tuning of hyperparamters and more efficient use of the Self-SL trained weights, Self-SL should bring consistent benefits for all cases where not most/all of the dataset is labeled.\\
    Another advantage is the comparatively fast training, shorter than half of the amount of training time than that of models with basic schedule. This should also allow to train more models and faster as soon as "good representations" are obtained.\\
    An alternative to Self-SL pretraining or one which could be used in combination would be transfer leraning by using models pre-trained on other datasets which have been shown to show great success and is the de-facto standard in NLP with models like BERT.
    \item Sem-SL performed in our setting very well on the dataset CIFAR-10 and also was the best performing training strategy for CIFAR-10 LT and performed as well as Self-SL models.\\
    However, on CIFAR-100 the performance with our shorter training and the ResNet-18 significantely degraded the performance from the values results in the paper and on MIO-TCD and ISIC-2019 we barely outperformed the basic models.\\
    This could possibliy be due to a wrong choice in hyperparameters but we swept the values noted as most important in the paper and changed the models to be better able to handle imbalanced data.\\
    This unsureness and hardness of training these models in combination with their very long training time (factor 40 to 80) compared to a standard training and the hardness of evaluating the performance as noted by  \cite{oliverRealisticEvaluationDeep2019} led us to omit results for AL on MIO-TCD and ISIC-2019 entirely.
    Based on this we recommend users with access to limited computing ressources not to run Sem-SL baselines and instead focus on Self-SL and finetuning basic models.
\end{itemize}
\paragraph{Realistic Method Configurations}
\begin{itemize}
    \item Our strategy of tuning hyperparameters with a reduced searchspace on only the first AL iteration leads to a signifantely reduced cost in optimization compared with optimizing every iteration, 
    while outperforming all other methods and performing on par/better than \cite{munjalRobustReproducibleActive2022a}.
    \item Using proper hyperparameters and especially Dataaugmnetation for our Basic models led to an improvement of performance comparable with five times as much data (see MIO-TCD, ISIC-2019 -- check CIFAR-X).
    \item For Self-SL models the hypeparameters showed not to be the most crucial parameter, mostly the effective utilization of representations for the optimization was necessary -- especially in the low-label regime.
    \item For Sem-SL models the parsing of hyperparameters proved to be challenging due to the extremely high training cost compared to Self-SL and Sem-SL. (Note which parameters were important!)\\
    \item A combination of Sem-SL and Self-SL as described in \cite{} [TODO] was experimented with but did not lead to satisfactory results in our experiments on CIFAR-10 and was therefore not further investigated.\\
    However, we deem this venue to be highly interesting for further research. Especially since Self-SL pretrained models should have to potential to significantely speed up Sem-SL training schedules.
\end{itemize}
\paragraph{Realistic Data Scenarios}
\begin{itemize}
    \item AL seems to improve upon random the most for class imbalanced data, when seen as effective per label.\\ Reverse argument: Random strategy suffers the most from imbalanced data.
    \item AL performance is greatly dependent upon initial budget and acquisition size (especially for low label) -- medium label would require further experiments.
    \item The validation set sizes we compared did not often lead to great changes in performance (compare random values)
\end{itemize}
\subsection{Key Take-Aways}
\paragraph{When does Active Learning bring benefits?}
We will focus now on settings where AL brings benefits (and is worth the additional effort over random sampling...).
Since as our experiments show that AL by no means is robust all-round approach which can be used without a recipe.
To be more exact, here we note: When do the AL strategies which we benchmarked with our exact experimental settings bring benefits.
\begin{itemize}
    \item For balanced datasets in the high label (and regardless of acq size \cite{munjalRobustReproducibleActive2022a} and method) regime for both Self-SL and Basic Models.\\
    However, it seems counterintuitive that AL is most generally useful in the case where each individual additional sample leads to the smalles increase in performance.
    \item For imbalanced datasets AL with some form of explorative strategy (Core-Set and BatchBALD) is beneficial across all label regimes, especially in combination with small acquisition sizes.\\ 
    (We deem this setting to be more generally applicable since when is it actually known that the acquired dataset is rougly equally distributed if it has not been sighted before? -- working with minimal information here and both datasets conisisting of real-world acquired data with minimal filtering are heavily imbalanced.)
    \begin{itemize}
        \item Cold-Start for Self-Supervised Pre-Trained model the bad performance of BALD seemed to be highly counterintuitive, but based on these experiments we believe to have shown a way to handle the Cold-Start for good performing models.\\
        Namely by making use of the performance of the model with uncertainty based acquisition methods and reducing the acquisition size (or simulating this with BatchBALD and therefore enforcing diversity).\\
        As to be expected an explorative query strategy such as Core-Set does not suffer from the Cold-Start as much as an uncertainty based strategy such as BALD or Entropy, however it does not make optimal use of the model performance and desicision boundary except for its representations.\\
        Further an explorative strategy such as K-Center Greedy based Core-Set may suffer from oversampling from the tails of the distribution. This, however, could be improved by using another approach for the K-Center problem.\\
    \end{itemize}
    \item Acquisition Size has to be set properly and is an important factor in the low (\& medium) label regime, especially if the model-performance is not the reason for the Cold-Start problem.
    \item Hyper-Parameter Tuning and Good training strategies are more important than AL strategy for final model performance and bring clear gains.
\end{itemize}
\subsection{Interesting Directions}
Using ensembles of Pre-Trained models obtained with K-Fold CV. High validation set size was mostly implemented to finetune Sem-SL.
This should give access to Ensembles for Bayesian Learning and generally better uncertainty values, but it does complicate latent spaces approaches like Core-Set.\\
Strategies which combine explorative and uncertainty based metrics seem to be highly interesting when finetuning pre-trained models.
This seems to be beneficial for both allowing the use of AL and significantely improving the performance and stabilizing the optimization problem of learning the classsifier.
Since generally the optimal hyperparameters for finetuning the pre-trained models did not change much (at all with significant differences) compared to the basic models.\\
A note on acquisition size: many papers try to use the biggest acquisition size as possible to minimize training cost and Mechanical Turk labeling \cite{atighehchianBayesianActiveLearning2020}.
We, however, believe that AL in combination with fast and realiable ML algorithms could be run in the background fast and iterative while labeling -- making AL more applicable under a wider variety of settings.
This is especially interesting to allow end-users to use deep learning to solve their own classification problems and the end-goal is not a dataset, but one relatively well function model that can be used to solve a specific task.
Allowing to use ML in research for tasks where currently no large labeled datasets exists, but big unlabeled datasets.

\subsection{Conclusion}
What changes do we believe does current AL research require to better reflect the wide variety of different settings under which AL will have to operate consistently 
Our recommendations for evaluating and developing Active Learning experiments go as follows:
\begin{itemize}
    \item AL should always be evaluated in combination with Self-SL and/or pre-trained models, since these are cheap and easy baseline models with strong indication for significant performance boosts.
    \item AL should be evaluated and developed on different datasets and label regimes to reduce the risk of overfitting to the evaluation dataset and give clear instructions on how to roll out/set hyperparameters if used on a new dataset.\\
    The whole point is that AL should be able to transfer to novel and unsighted datasets. Therefore they have to generalize with minimal knowledge.
    More specifically they should be evaluated and developed as follows with the goal of outperforming random choice under these settings:
    \begin{itemize}
        \item Different Label Regimes with a focus on the low data regime 
        \item Different Datasets both with and without imbalances and different performance metrics (F1, balanced Accuracy etc.) (medical domain)
    \end{itemize}
    \item Hyperpameters of models should be selected using a clear training validation split, it is simply unrealistic to not do that at all.
\end{itemize}
Our findings indicate towards settings where AL is most likely the right choice for practitioners:
\begin{itemize}
    \item Settings with an abundance of labeling budget and a big initial labeld dataset.
    \item When Self-SL provides benefits, then small acquisition sizes with BALD and/or BatchBALD /(Core-Set) can be applied for bigger acquisition sizes.
    \item Settings for which a high class imbalance is to be expected, but a balanced classifier is the end goal.
\end{itemize}



==> tex/99_depr_tex/07_OLD_conclusion.tex <==


% Add statement about AL in generally with bet and talk about costs
% Add general conclusions
% The general trend is that in later stages AL brings benefits. However in practice someone does not know at which stage on is currently due to the validation paradoxon (K2).
If the practical question arises whether or not to employ AL on a novel specific dataset we propose to formulate it as a bet which goes as follows:
"If AL is employed in practice one bets computational effort and setup cost against a performance increase over random queries (expected gain) with an unknown outcome".
Where the gain should lead to a reduction of labeling cost.
However, by careful evaluating AL methods the `expected gain' can be estimated if it is evaluated under enough different conditions and is in the best case-scenario generally higher than the cost if it is a well generalizing method (working out-of-the-box).
\\
% First, we would like to offer a to our knowledge novel interpretation of AL:\\
% AL is essentially a wager against random sampling, where the practitioner wagers computational effort and setup cost, in the hope of reducing labeling cost by outperforming random queries. \\
Using this interpretation of AL we derived our main findings which we already presented in \cref{sec:intro} and will now give our final conclusion:
% we will draw our final conclusions here and also our main findings were derived with this thought process.
Generally the goal of AL research in our opinion should be to offer practitioners an `informed choice' with regard to computational effort, setup cost and expected gain.
With our empirical study and proposed improvements of the evaluation protocol we hope to shed a light on the expected gain especially with regard to our key-parameters and the explored QMs which are summarized in \cref{sec:intro}.
Our recommendations for evaluating AL methods goes as follows to estimate the `expected gain' as accurately as possible:
\begin{itemize}
    % K1
    \item AL method development should follow a strict setup with developmental datasets for recipe optimization (including HPs) and roll-out datasets strictly used for evaluation with varying class distributions and dataset complexities.
    % K2 + K3 
    \item AL methods should be evaluated with regard to Query Size and Starting Budget to simulate different real-world environments or give a clear instructions for setting them to obtain a high expected gain.
    % K4
    \item HPs of all methods used should be carefully optimized for each dataset based on clear heuristics, especially the classifier since it is the measurement tool for performance of AL methods.
    % K5
    \item AL should be evaluated in combination with and against Self-SL (\& Semi-SL) since gains obtained with training strategies over ST can be confirmed on a validation set.
\end{itemize}
Our recommendations for using AL in practice are also a direct result of the proposed wager.
In short, if the expected gain can be estimated to be smaller than the expected cost of.
Therefore, delevopment should be directed towards minimizing the expected wager cost:
\begin{itemize}
    \item Development effort should be directed towards making AL an easy to use tool to reduce setup cost thereby `reducing the wager of AL' potential practitioners face.
    \item Methods reducing training time s.a. Self-SL in combination with AL is also a promising direction since it reduces computation effort
    % and potentially offers smaller query sizes since training time was the major contributor to computation cost in our study with the exception of the BatchBALD QM. 
    This potentially increases the `excpected gain of AL`, especially in low-label settings.
    % oved to increased the `excpected gain of AL` in the low-label setting from a negative to a postive.
\end{itemize}
% Our recommendations for using AL in practice are also a direct result of the proposed wager.
% In short, if the expected gain can be estimated to be smaller than the expected cost of the bet.

More specifically we would like to highlight the following settings indicating a benevolent cost to gain ratio based on our empirical evidence:
\begin{itemize}
    \item Settings with high labeling cost, since it allows to use small query sizes and initial budgets and neglect training cost (high cost where already small gains leads to substantial benefit).
    % this induces cost s.a. medicine
    \item Settings with low labeling cost, by using large query sizes and large budgets leading to a small training cost (small cost and small expected gain).
    \item Settings with datasets where a mismatch between class distribution and importance is to be expected increasing the expected gain.
\end{itemize}





%%%%%%%%%%%%%%%% OLD Version %%%%%%%%%%%%%%%
% \paragraph{When should I consider applying AL on my task?} 

% \begin{itemize}
%     \item Settings with an abundance of labeling budget and a big initial labeled dataset.
%     \item If Self-SL provides benefits, then small acquisition sizes ($~50$ observations) with BatchBALD or Core-Set can be applied for bigger acquisition sizes.
%     \item Settings for which a high class imbalance is to be expected, but a balanced classifier is desired.
% \end{itemize}
% % Write about cost benefit.
% Therefore a useful interpretation of AL would be a bet with its properties: Using it leads in a good outcome to a gain in performance over random or in a very bad scenario to a loss in performance. 
% Since the case of a loss of performance should be avoided at all cost due to additional cost of AL over random sampling, we interpret the results of AL in this manner.
% Across all experiments the explorative Core-Set QM brought most consistently gains over random sampling.\\
% In some cases (especially high-label regime) the uncertainty based QMs significantely outperformed Core-Set with BALD being more robust than Entropy.\\
% Entropy had many instances with significantely worse performance than random queries.\\
% Therefore a QM combining both paradigms of uncertainty reduction and exploration shows strong potential as superior QM.

% Our experiments provide strong evidence that the standard evaluation practice for AL is unrealistic and that an AL pipeline encompasses much more than purely the selection of a proper QM. 
% %So what changes do we believe does current AL research require to better reflect the wide variety of different settings under which AL will have to operate consistently?
% %Our recommendations for evaluating and developing Active Learning experiments go as follows:
% \paragraph{How to best set up an AL system?} Therefore we believe, that current AL requires a better reflection of the wide variety of different settings under which AL will have to operate consistently. We formulate our recommendations for evaluating and developing AL experiments along these lines:
% \begin{itemize}
%     \item AL should always be evaluated in combination with Self-SL and/or pre-trained models, since these are cheap and easy baseline models with strong indication for significant performance boosts.
%     \item AL should be developed and evaluated on different datasets with multiple label regimes to reduce the risk of overfitting to the development dataset and settings. These datasets should cover: varying label distributions, different dataset complexities and different label regimes (4. different imaging modalities).
%     \item New introduced AL methods should give clear instructions on how to set it up with regard to the key-parameters discussed in this work (\& especially parameters of the QM) allowing to roll them out on a new datasets and show robustness on multiple datasets or follow our proposed evaluation protocol with multiple label regimes on multiple datasets to verify robustness.
%     \item Hyperparameters of models should be selected using a clear validation set or inferred by rules which do not follow the lines of implementation and hyperparameters based on the whole dataset!
%     \item Development effort should be directed towards making AL an adaptable toolbox which can easily rolled out to novel datasets to make utilizng AL as cost efficient as possible instead of the current focus on novel QMs improving over partly badly fine-tuned SotA models since it is questionable whether these results can be reproduced with better models. This development either forces everyone to re-implement and rerun all experiments with their own setting or not properly allowing them to compare themselves with the current literature.
%     % \item Different Datasets
%     % The whole point is that AL should be able to transfer to novel and unsighted datasets. Therefore they have to generalize with minimal knowledge.
%     % More specifically they should be evaluated and developed as follows with the goal of outperforming random choice under these settings:
%     % \begin{itemize}
%     %     \item Different Label Regimes with a focus on the low data regime 
%     %     \item Different Datasets both with and without imbalances and different performance metrics (F1, balanced Accuracy etc.) (medical domain)
%     % \end{itemize}
%     % \item Hyperpameters of models should be selected using a clear training validation split, it is simply unrealistic to not do that at all.
% \end{itemize}
% Our findings indicate towards settings where AL is most likely the right choice for practitioners:
% \begin{itemize}
%     \item Settings with an abundance of labeling budget and a big initial labeled dataset.
%     \item If Self-SL provides benefits, then small acquisition sizes ($~50$ observations) with BatchBALD or Core-Set can be applied for bigger acquisition sizes.
%     \item Settings for which a high class imbalance is to be expected, but a balanced classifier is desired.
% \end{itemize}

% % \subsection{Interesting Directions}
% % Using ensembles of Pre-Trained models obtained with K-Fold CV. High validation set size was mostly implemented to finetune Sem-SL.
% % This should give access to Ensembles for Bayesian Learning and generally better uncertainty values, but it does complicate latent spaces approaches like Core-Set.\\
% % Strategies which combine explorative and uncertainty based metrics seem to be highly interesting when finetuning pre-trained models.
% % This seems to be beneficial for both allowing the use of AL and significantely improving the performance and stabilizing the optimization problem of learning the classsifier.
% % Since generally the optimal hyperparameters for finetuning the pre-trained models did not change much (at all with significant differences) compared to the basic models.\\
% % A note on acquisition size: many papers try to use the biggest acquisition size as possible to minimize training cost and Mechanical Turk labeling \cite{atighehchianBayesianActiveLearning2020}.
% % We, however, believe that AL in combination with fast and realiable ML algorithms could be run in the background fast and iterative while labeling -- making AL more applicable under a wider variety of settings.
% % This is especially interesting to allow end-users to use deep learning to solve their own classification problems and the end-goal is not a dataset, but one relatively well function model that can be used to solve a specific task.
% % Allowing to use ML in research for tasks where currently no large labeled datasets exists, but big unlabeled datasets.
